Automatic Detection of Five API Documentation Smells: Practitioners' Perspectives

The learning and usage of an API is supported by official documentation. Like source code, API documentation is itself a software product. Several research results show that bad design in API documentation can make the reuse of API features difficult. Indeed, similar to code smells or code antipatterns, poorly designed API documentation can also exhibit 'smells'. Such documentation smells can be described as bad documentation styles that do not necessarily produce an incorrect documentation but nevertheless make the documentation difficult to properly understand and to use. Recent research on API documentation has focused on finding content inaccuracies in API documentation and to complement API documentation with external resources (e.g., crowd-shared code examples). We are aware of no research that focused on the automatic detection of API documentation smells. This paper makes two contributions. First, we produce a catalog of five API documentation smells by consulting literature on API documentation presentation problems. We create a benchmark dataset of 1,000 API documentation units by exhaustively and manually validating the presence of the five smells in Java official API reference and instruction documentation. Second, we conduct a survey of 21 professional software developers to validate the catalog. The developers agreed that they frequently encounter all five smells in API official documentation and 95.2% of them reported that the presence of the documentation smells negatively affects their productivity. The participants wished for tool support to automatically detect and fix the smells in API official documentation. We develop a suite of rule-based, deep and shallow machine learning classifiers to automatically detect the smells. The best performing classifier BERT, a deep learning model, achieves F1-scores of 0.75 - 0.97.

==> DocBotSANER2021 (Camera Ready)/backup/study_result_backup.tex <==
\section{Automatic Detection of The Smells}
We answer the following four research questions:

\begin{enumerate}[label=RQ\arabic{*}., leftmargin=25pt]
  \item How accurate are rule-based classifiers to automatically detect the documentation smells?
  \item Can the shallow machine learning models outperform the rule-based classifiers?
  \item Can the deep machine learning models outperform the shallow learning models?
  \item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}
\subsection{Performance Metrics}
We analyze and report the performance of each of the techniques developed and experimented as part of the algorithms development steps. We used 5-fold iterative stratified cross-validation for reporting performances that has been recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}. We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

\begin{inparaenum}[(a)]
\item\bf{Iterative Stratified Cross-Validation}
Traditional $k$-fold cross-validation is a statistical method of evaluating machine learning algorithms which divides data into $k$ equally sized folds and runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each iteration, each of the $k$ folds is used as the held-out set for validation while the remaining $k-1$ folds are used as training sets. Stratified cross-validation is used to make sure that each fold is an appropriate representative of the original data by producing folds where the proportion of different classes is maintained \cite{stratified_cross_validation_paper}. However, stratification is not sufficient for multi-label classification problems as the number of distinct labelsets (i.e., different combinations of labels) is often quite large. For example, there can be 32 combinations of labels in our study as there are 5 types of documentation smells. In such cases, original stratified $k$-fold cross-validation is impractical since most groups might consist of just a single example. Iterative stratification, proposed by \cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy approach of selecting the rarest groups first and adding them to the smallest folds while splitting. Hence, we used this iterative stratified cross-validation in our experiment. 

\item\bf{Exact Match Ratio}
In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

\begin{equation}
EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
\label{eq:EMR}
\end{equation} %&

{$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
}


\item\bf{Hamming Loss}
Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
\begin{equation}
HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
\end{equation}

{$N$ is the total number of data, $L$ is the total number of labels.}

\item\bf{Accuracy}
Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
\begin{equation}
A = \frac{TP+TN}{TP+FN+TN+FP}
\label{eq:acc}
\end{equation}

{$TP$ is the number of true positives, $FN$ is the number of false
negatives, $FP$ is the number of false positives, $TN$ is the number of true
negatives.}


\item\bf{Precision}
Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
\begin{equation}
P  = \frac{TP}{TP+FP} 
\label{eq:precision}
\end{equation} %&


\item\bf{Recall}
Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

\begin{equation}
 R = \frac{TP}{TP+FN}
 \label{eq:recall}
 \end{equation} 
 

\item\bf{F1-score}
F1-score is the harmonic mean of precision and recall.
\begin{equation}
F1 = \frac{2\cdot P\cdot R}{P+R}
\label{eq:f-score}    
\end{equation}

\end{inparaenum}

\subsection{ How accurate are rule-based classifiers to automatically detect the documentation smells? (RQ1)}
\subsubsection{Rule-based Metrics}
%\subsubsection{Approach}
%\gias{discuss the studied features, put the feature summaries in a table}
%discuss the features, group the features into a set of feature dimensions.


\begin{inparaenum}[(a)]
\item\bf{Documentation Length.} We use the length of every documentation in order to capture the extensiveness of the bloated documentations.

\item\bf{Readability Metrics.} We measure Flesch readability metrics for the documentations and use them as a feature to analyze the understandability of documentation. This feature might be useful to detect tangled documentations.

\item\bf{Number of Acronyms and Jargons.} Since acronyms and jargons increase the complexity of a reading passage, we use the number of acronyms and jargon in every documentation to detect the tangled documentation by estimating the understandability.

\item\bf{Number of URLs.} As URLs are hints of possible fragmentations in the documentation, we use the number of URLs to capture these smells.

\item\bf{Number of function, class and package name mentioned.} We use the number of functions, classes, packages mentioned in documentation to capture excess structural information and fragmentation.

\item\bf{Edit Distance.} From the definition of lazy documentation, it can be said that the edit distance of a lazy documentation and its’ unit definition (method prototype) will be comparatively small. So we calculate the edit distance between the documentation description and method prototype and use it as a feature for our machine learning models.

\item\bf{Average Cosine Similarity.} We calculate the avg. cosine similarity of the documentations’ description. For this, we calculate the cosine similarities between each possible pair of that documentation and take their avg value for normalization. This feature will help to detect redundancy in the documentations.
\end{inparaenum}

\subsubsection{Results}
discuss the results by varying the metric thresholds

\subsection{How accurate are shallow machine learning models to automatically detect the documentation smells? (RQ2)}
\subsubsection{Shallow Learning Models}
We applied both traditional and deep learning algorithms to detect documentation smells. We employed different decomposition approaches (i.e., One-Vs-Rest, Label Powerset, Classifier Chains)~\cite{multilabel_decomp_1_MultilabelClassificationAnOverview,multilabel_decomp_2_AReviewOnMultilabelLearning,multilabel_decomp_3_ATutorialOnMultilabelClassification,multilabel_decomp_4_LearningFromMultilabelData} with Support Vector Machine (SVM) \cite{SVM_SupportVectorNetworks} as the base estimator for multi-label classification of documentation smells. We chose SVM since it has been successfully used with these decomposition approaches for multi-label classification in previous studies \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}. SVM has also shown great performance in text classification tasks \cite{svm_text_classification_1, svm_text_classification_2}. We also evaluated adapted approaches like ML-$k$NN \cite{MLkNN_ALazyLearningApproach}, and deep learning models like Bi-LSTM \cite{bi_lstm_BidirectionalRecurrentNeuralNetworks}, and BERT \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. 

%\subsubsection{OVR-SVM}
%\label{subsubsec:ovr_svm}
\begin{inparaenum}[(a)]
\item\bf{One-Vs-Rest} is a heuristic method that works by decomposing the multi-label classification problem into multiple independent binary classification problems (one per class) \cite{multilabel_decomp_1_MultilabelClassificationAnOverview, multilabel_decomp_3_ATutorialOnMultilabelClassification}. It trains a single classifier per class, with the samples of that class as positive samples and all other samples as negatives. All the independent classifiers then separately give individual class predictions for unseen data. We evaluated One-Vs-Rest (OVR) approach with SVM (as the base estimator) for detecting documentation smells. One-Vs-Rest support vector machine (OVR-SVM) has been successfully applied in several problems \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM, multilabel_decomp_1_MultilabelClassificationAnOverview}. We used RBF kernel for the SVM classifiers as recommended by earlier works \cite{svm_rbf_1_AComparisonStudyOfDifferentKernelFunctions, svm_rbf_2_APracticalGuideToSVM}.

%\subsubsection{LPS-SVM}
%\label{subsubsec:lps_svm}
\item\bf{Label Power Set (LPS)} treats every combination of labels as a new class and approaches in a multiclass classification manner \cite{LearningMultiLabelSceneClassification}. As a result, this method has high computational complexity. However, it is capable of taking label correlation into account. We used SVM (with RBF kernel) as the base estimator of the Label Power Set method \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}.


%\subsubsection{CC-SVM}
%\label{subsubsec:cc_svm}
\item\bf{Classifier Chains (CC)} constructs a chain of binary classifiers, where every classifier uses the predictions of all the previous classifiers of the chain \cite{CC_1_ClassifierChainsForMultilabel, CC_2_ClassifierChainsForMultilabel}. This way the method can take label correlations into account. We constructed a Classifier Chain (CC) of SVMs and evaluated its’ performance for documentation smell detection.



%\subsubsection{ML-$k$NN}
%\label{subsubsec:ml_knn}
\item\bf{Multi-label $k$ Nearest Neighbors (ML-$k$NN)} is derived from the traditional $k$-nearest neighbor ($k$NN) algorithm \cite{MLkNN_ALazyLearningApproach}. It finds the $k$ nearest neighborhood of an input instance using $k$NN, then uses Bayesian inference to determine the label set of the instance. We studied this method because it has been reported to achieve considerable performance for different multi-label classification tasks in previous studies \cite{MLkNN_ALazyLearningApproach, mlknn_MultilabelTextClassificationUsingSemanticFeatures}. We used ML-$k$NN with the number of nearest neighbors, $K$ = 10 during our experiment as recommended by \cite{mlknn_MultilabelTextClassificationUsingSemanticFeatures}.

\end{inparaenum}

\subsubsection{Studied Features} In this subsection, we describe the features that we used to train our SVM and \it{k}NN-based models (see section \ref{subsubsec:ovr_svm} to \ref{subsubsec:ml_knn}) for documentation smell detection.

use two types of features: the rule-based metrics, bag-of-words (as a proxy of word embeddings which will be used in BERT/LSTM - you need to 
ensure that reviewers are convinced that you have looked at each option before claiming BERT is a the best classifier)

%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}

Table \ref{table_overall_performance} represents the performance of the ML models for detecting documentation smell as a multi-label classification problem. We observe that OneVsRest (OVR) and Classifier Chain (CC) achieved equal results. CC-based models are generally superior to OVR-based models because of the capability of capturing label correlation. Since the labels (types) of the documentation smells are not correlated, the CC-based SVM could not exhibit higher performance than the OVR-based SVM. However, Label Powerset (LPS) achieved lower performance than the OVR and CC-based models. To show better results, LPS-based SVM would require sufficient instances for all 32 classes of 5 smell types. Deep learning-based models like Bi-LSTM and BERT, on the other hand, outperformed the SVM and $k$NN-based models by achieving higher exact match ratios. Although Bi-LSTM showed higher Hamming loss, BERT achieved similar to the SVM and $k$NN-based models. Therefore, in terms of Hamming loss, deep learning-based models did not show any improvement. However, considering both exact match ratio and Hamming loss as the performance metrics, we can deduce that BERT is the most suitable of all the models experimented in detecting the documentation documentation smell.
\begin{table}[t]
\caption{Shallow models on the overall smell types detection}
\centering
%\begin{center}
%\scalebox{1.0}
%\resizebox{\columnwidth}{!} %new add
%{
%\renewcommand*{\arraystretch}{2}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule
\textbf{Rule-based} & .17                        & .35       \\ %\hline
\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
%\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
%\textbf{BERT}    & \textbf{.84}               & .15                   \\ 
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
\bottomrule
%{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
%{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
%\hline
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}
Table \ref{table_individual_performance} shows the performance of the ML models
on each type of documentation smells. Although SVM and $k$NN-based models
achieved slightly better accuracy than Bi-LSTM and BERT, the later models
outperformed SVM and $k$NN-based models in F1-score. This behavior is due to the
unequal distribution of the smell types over the dataset. SVM and $k$NN-based
models produced more false-negative results because the number of positive
instances for an individual smell type is significantly lower than the number of
negative instances for that type. As a result, SVM and $k$NN-based models showed
quite low recalls for some types (Excess Struct, Tangled, and Fragmented) and
consequently resulted in low F1-scores. 
%\subsubsection{Feautre Importance Analysis}
\gias{TODO: do the feature-based analysis here, i.e., ablation study on the shallow learning models as discussed}

\subsection{Can the deep machine learning models outperform the shallow learning models? (RQ3)}
\subsubsection{Deep Learning Models}
%\subsubsection{Bi-LSTM}
Bidirectional LSTM is more capable of exploiting contextual information than the unidirectional LSTM \cite{bilstm_FramewisePhonemeClassificationWithBiLSTM}. Hence, the Bi-LSTM network can detect the documentation smell by capturing the information of the API documentations from both directions. We constructed a Bi-LSTM model with 300 hidden states and initialized it using the pre-trained GloVe embedding \cite{Glove_GlobalVectorsForWordRepresentation} of 100 dimensions. We used ADAM optimizer \cite{adam_optimizer} with an initial learning rate of 0.001. We trained the model with batch size 256 over 10 epochs.


%\subsubsection{BERT}
Considering the great success of BERT (Bidirectional Encoder Representations from Transformers) in various natural language processing and text classification tasks \cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}, we feel motivated to evaluate its’ performance in documentation smell detection. BERT is a  pre-trained model which was designed to learn contextual word representations of unlabeled texts \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. We used BERT-Base for this study which has 12 layers with 12 attention heads and 110 million parameters. We trained it on our labeled dataset for 10 epochs with a mini-batch size of 32. We used early-stop to avoid overfitting \cite{early_stop_bert_1} and considered validation loss as the metric of the early-stopping \cite{early_stop_bert_2}. The maximum length of the input sequence was set to 256. We used AdamW optimizer \cite{adam_w} with the learning rate set to 4e\textsuperscript{-5}, ß1 to 0.9, ß2 to 0.999, and epsilon to 1e\textsuperscript{-8} \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers, bert_fine_tuning}. We used binary cross-entropy to calculate the loss \cite{binary_cross_AreLossFunctionSame}. 


\subsubsection{Studied Features} talk about word-embeddings

\subsubsection{Results}
On the other hand, Bi-LSTM and BERT
focused on capturing generalized attributes for each smell type and as a result,
achieved impressive performance in all the performance metrics. Overall, BERT
showed promising results among all the models in accurately detecting each of
the individual documentation smells.
\begin{table}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule

%\textbf{Rule-based} & .17                        & .35       \\ %\hline
%\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
%\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
%\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
%\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
\textbf{BERT}    & \textbf{.84}               & .15                   \\ %\hline
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}

% \begin{table*}[!ht]
% \caption{Performance on different type of documentation smells}
% \begin{center}
% \scalebox{1.0}
% {
% %\renewcommand*{\arraystretch}{3}
% \begin{tabular}{ccccccccccccccccccccc}
%                                        & \multicolumn{20}{c}{}                                         \\ \cline{2-21} 
%{}                  & \multicolumn{4}{c|}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c|}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c|}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c|}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c|}{\textbf{Fragmented}}                                                                  \\ \hline
% {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ \hline
% %{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
% %{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
% %{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
% %{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
% %{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
% {\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
% {\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ \hline
% \end{tabular}
% }
% \label{table_individual_performance}
% \end{center}
% \end{table*}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
\bottomrule
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
\gias{TODO. Now report some misclassified cases of BERT per documentation smell and explain why the misclassification occurred.}

\subsection{Can the detection of one documentation smell support the detection another smell? (RQ4)}
In multi-label learning, the labels might be interdependent and correlated \cite{label_correlation_paper_1}. We used Phi Coefficients to determine such interdependencies and correlations between different documentation smells. The Phi Coefficient is a measure of association between two binary variables \cite{phi_coefficient_paper}. It ranges from -1 to +1, where ±1 indicates a perfect positive or negative correlation, and 0 indicates no relationship. We report the Phi Coefficients between each pair of labels in Figure \ref{fig:label_correlation}. We find that there is almost no correlation between `Fragmented’ and any other smell (except `Lazy’). By definition, the information of fragmented documentation is scattered in many sections or pages. Hence, it has little to do with smells like `Bloated’, `Excess Structural Information’, `Tangled’. We also observe that there is a weak positive correlation (+0.2 to +0.4) among the `Bloated’, `Excess Structural Information’, and `Tangled’ smells. One possible reason might be that if a documentation is filled with complex and unorganized information (Tangled), and unnecessary structural information (Excess Structural Information), it might be prone to become bloated as well. On the other hand, `Lazy’ smell has a weak negative correlation (-0.2 to -0.3) with all other groups since these kinds of documentation are often too small to contain other smells. However, none of these coefficients is high enough to imply a strong or moderate correlation between any pair of labels. Hence, it justifies our catalog by indicating that all the smells that we proposed are sufficiently unique in nature.

\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
   \hspace*{-.7cm}%
  \includegraphics[scale=.5]{new_images/label_correlation.png}
 % \vspace{-4mm}
  \caption{Correlation of different documentation smells. Red, Blue, and Gray mean positive, negative, and no correlation respectively. Intensity of color indicates the level of correlation.}

  \label{fig:label_correlation}
%\vspace{-4mm}
\end{figure}


% 
% \subsection{Ablation Study (RQ4)}
% BERT - epoch change
% SVM - feature change.



%\subsection{How accurate is each feature dimension?}
%answer RQ

%\subsection{How well does hypertuning work in the ML models?}
%answer RQ.


==> DocBotSANER2021 (Camera Ready)/benchmark.tex <==
\section{A Benchmark of API Documentation Smells}\label{sec:benchmark}
We describe the methodology to create our benchmark of API documentation smells (\sec\ref{sec:benchmark_method}) and then present the 
benchmark with real-world examples (\secs\ref{sec:five_doc_smells} - \ref{sec:benchmark-details}).
\subsection{Benchmark Creation Methodology}\label{sec:benchmark_method}
\begin{figure}[t]
\centering
	\centering
   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
   	\includegraphics[scale=.85]{images/workflow_mod4}
   	\caption{The three major steps in benchmark creation process.}
   	 \label{fig:MethodologyOverallBenchmark}
\vspace{-5mm}
\end{figure}
Code and design smells are relatively well studied fields of software engineering. However, to the best of our knowledge, 
this is the first research on API documentation smells. As such, 
we needed to investigate both the literature 
on API documentation~\cite{Aghajani-SoftwareDocPractitioner-ICSE2020,Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Uddin-HowAPIDocumentationFails-IEEESW2015,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a} 
and the diverse API documentation resources (e.g., Java SE docs) during the creation of our catalog of API documentation smells. 
We followed a three-step process, which closely mimics the standard approaches followed in 
code/design smell formulation studies~\cite{Abidi-AntiPatternMultiLanguage-EuroPLoP2019,Abidi-CodeSmellsMultiLanguage-EuroPLoP2019}.  
The three steps are outlined in \fig\ref{fig:MethodologyOverallBenchmark} and are explained below.  

\nd\bf{Knowledge Acquisition.} Similar to code and design smells that do not directly introduce a defect or a bug into a software system, documentation smells refer to
presentation issues that do not make a documentation incorrect, rather they hinder its proper usage due to the lack of quality in the design 
of the documented contents. As such, we studied extensively the API documentation literature that reported issues related to API documentation presentation and usability~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019}.  
For example, the most recent paper on this topic was by Aghajani et al.~\cite{Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Aghajani-SoftwareDocPractitioner-ICSE2020}, who 
divided the `how' problems in API documentation into four categories: maintainability (e.g., lengthy files), readability (e.g., clarity), 
usability (e.g., information organization like dependency structure), and usefulness (e.g., content not useful in practice). Previously, Uddin and Robillard~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015} 
studied 10 common problems in API documentation by surveying 323 IBM developers. They observed four common problems related to presentation, i.e., bloated (i.e., too long description), 
tangled (complicated documentation), fragmented (i.e., scattered description), and excessive structural information (i.e., information organization like dependency structure).
Given that the four problems appeared in both studies, we included each as a documentation smell in our study. In addition, we added lack of 
proper description of an API method as a `lazy' documentation smell, because incomplete documentation problems are 
discussed in literature~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocPractitioner-ICSE2020} as well as in online developer discussions  (see \fig\ref{fig:motivating_lazy_example}).  
\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
   \hspace*{-.7cm}%
  \includegraphics[scale=.16]{images/lazy.JPG}
 % \vspace{-4mm}
  \caption{Tweet complaining about lazy documentation of API method.}

  \label{fig:motivating_lazy_example}
\vspace{-2mm}
\end{figure}

\nd\bf{Feasibility Analysis.} Once we decided on the five smells, we conducted a feasibility study by looking for real-world examples of the smells in official
and instructional API documentation. This was important to ensure that the smells are prevalent in API documentation and that we can find those with reasonable confidence, because otherwise there is no way we can design automated techniques to detect those automatically. We combined our 
knowledge of the five smells gained from API documentation literature with active exploration of the five smells in the API official documentation. We conducted multiple 
focus group discussions where all the four authors discussed together by analyzing potential examples of the five smells in API documentation and by 
mapping the characteristics of such API documentation with the description of the smells in the literature/developer discussions. Before every such 
focus group meeting, the first two authors created a list of 50 API documentation units with their labels of the five smells in the units. The four authors 
discussed those labels together, refined the labels, and identified/filtered the labeling criteria. This iterative process led to increased understanding 
among the group members on the specific characteristics of the five documentation smells. From multiple discussion sessions, 
the final output was a list of 50 labeled datapoints.    

\nd\bf{Benchmark Creation.} In the last step of the benchmark creation process, we expanded our 
initial list of 50 API documentation units with smell labels as follows. 
We collected documentations of over 29K methods belonging to over 4K classes of
217 different packages. We extracted these documentations from the online JAVA
API Documentation
website~\cite{website:javadocse7} through web
crawling and text parsing techniques. %\cite{web_crawl_book_1,web_crawl_book_2}.
%Then we created a benchmark dataset of 1000 labeled documentation. 
Since a documentation can contain multiple smells at the
same time, this is a multi-labeled dataset. We produced the benchmark as
follows. First, all the authors mutually discussed the documentation smells.
Then, we randomly selected 950 documentations from a total of 29K that we
extracted. Then the first two authors labeled the first 50 documentations
separately. When they finished, they consulted other co-authors and resolved the
disagreement based on the discussion. Then they continued with the next 50
documentations and repeated the same process. Their agreement of labeling has been
recorded using Cohen's Kappa Coefficient \cite{cohen_kappa_paper} for each
iteration, i.e., labeling 50 documentations (Table \ref{cohen_kappa_table}).
After the third iteration, both the authors reached a perfect
agreement level with Cohen’s Kappa Coefficient of $0.83$. Then they prepared a
coding guideline for the labeling task which was later presented to 17 
computer science undergraduate students. The students labeled the remaining 800
documentation units. During the entire coding sessions by the 17 coders, the first 
two authors remained available to them via Skype/Slack. Each coder consulted their labels with the two authors. 
This ensured quality and mitigated subjective bias in the manual labeling of the benchmark. 

% \begin{table}
% \centering
% \caption{Measure of agreement between two labelers.}
% \begin{tabular}{ccc}
% \toprule
% \textbf{\begin{tabular}[c]{@{}c@{}}\ \textbf{Iteration} \\   \textbf{No.}\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}\ \textbf{\# of} \\   \textbf{data}\end{tabular}} & 
% \textbf{\begin{tabular}[c]{@{}c@{}}\ \textbf{Cohen's Kappa} \\   \textbf{Coefficient}\end{tabular}} \\ \midrule
%  1 &  50                        & .49                   \\ %\hline
%  2 & 50               & .67                   \\ %\hline
%  3 & 50               & .83                   \\
% \bottomrule
% \end{tabular}
% %}
% \label{cohen_kappa_table}
% %\end{center}
% \end{table}

\begin{table}
\centering
\caption{Measure of agreement between two labelers}
\begin{tabular}{ccc}
\toprule
\textbf{Iteration ID}   &  \bf{Documentation Unit \#} & \bf{Cohen $\kappa$} \\ \midrule
 1 &  50                        & .49                   \\ %\hline
 2 & 50               & .67                   \\ %\hline
 3 & 50               & .83                   \\
\bottomrule
\end{tabular}
%}
\label{cohen_kappa_table}
%\end{center}
\end{table}

\subsection{The Five Documentation Smells in the Benchmark}
\label{sec:five_doc_smells}
%We describe the five API documentation smells using examples from our benchmark and provide summary statistics of the distribution of the smells in our benchmark.
%We provide examples of the five smells below.

\nd\bf{Bloated Documentation Smell.} By `Bloated’ we mean the documentation 
whose description (of an API element type) is verbose or excessively elaborate. 
It is difficult to understand or follow a lengthy documentation~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 
Moreover, it cannot be effectively managed that makes it hard to modify when needed, e.g., in case of any update in the API source code. 
In our benchmark, we found many documentations that are larger than necessary. 
For example, the documentation shown in \fig\ref{fig:bloated_example} is so verbose and lengthy that it is hard to follow and use it. Hence, it is a bloated documentation.   


%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Example Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]%[!htb]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  \includegraphics[scale=.48]{new_images/bloated_example.png}
 % \vspace{-4mm}
  \caption{Example of Bloated Smell.}

  \label{fig:bloated_example}
%\vspace{-4mm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%\anindya{Previously, at line 30, you mentioned "excessive" structure. Should it be consistent?}
\nd\bf{Excess Structural Information Smell.} Such a description of a documentation unit (e.g., method) 
contains too many structural syntax or information,
e.g., the Javadoc of the java.lang.Object class. Javadoc lists all the hundreds
of subclasses of the class. In our study, we find this type of documentation to
contain many class and package names. For instance, the documentation of \fig\ref{fig:excess_struct_example} contains many structural information (marked in
red rectangle) that are quite unnecessary for the purpose of understanding and
using the underlying method.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Example Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]%[!htb]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  \includegraphics[scale=.48]{new_images/excess_struct_example.png}
 % \vspace{-4mm}
  \caption{Example of Excess Structural Information.}

  \label{fig:excess_struct_example}
%\vspace{-4mm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%

\nd\bf{Tangled Documentation Smell.} A documentation of an API element (method) is `Tangled’ if it's
description is \it{tangled} with various information (e.g., from other methods). This makes it complex and
thereby reduces the readability and understandability of the description. \fig\ref{fig:tangled_example} depicts an example of tangled documentation which is
hard to follow and understand.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Example Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]%[!htb]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  \includegraphics[scale=.48]{new_images/tangled_example.png}
 % \vspace{-4mm}
  \caption{Example of Tangled Smell.}

  \label{fig:tangled_example}
%\vspace{-4mm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%



\nd\bf{Fragmented Documentation Smell.} Sometimes it is seen that the
information of documentation (related to an API element) is scattered (i.e., fragmented) over too
many pages or sections. In our
empirical study, we found a good number of documentation that contain many URLs
and references that indicate possible fragmentation smell. For example, the
documentation of \fig\ref{fig:fragmented_example} is fragmented as it refers
the readers to other pages or sections for details.
%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Example Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]%[!htb]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  \includegraphics[scale=.48]{new_images/fragmented_example.png}
 % \vspace{-4mm}
  \caption{Example of Fragmented Smell.}

  \label{fig:fragmented_example}
%\vspace{-4mm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%


\nd\bf{Lazy Documentation Smell.} We categorize a documentation as `Lazy’ if it contains very small information to convey to the readers. In many cases, it is seen that the documentation does not contain any extra information except what can be perceived directly from the function name. Hence, this kind of documentation does not have much to offer to the readers. We see a lazy documentation in \fig\ref{fig:lazy_example} where the documentation says nothing more about the underlying method than what is suggested by the prototype itself. 

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Example Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]%[!htb]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  \includegraphics[scale=.48]{new_images/lazy_example.png}
 % \vspace{-4mm}
  \caption{Example of Lazy Smell.}

  \label{fig:lazy_example}
%\vspace{-4mm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Distribution of API Documentation Smells in Benchmark}\label{sec:benchmark-details}

We calculated the total number of smells in our dataset (\fig\ref{fig:amount_of_multismell_in_dataset}). 
We found that  778 documentations (almost 78\%) of our dataset contain at least one smell. While most (524) of the smelly documentations contain only one type of smell, a small number (19) of documentations show as high as four smells at the same time. We also determined the distribution of different smells in our dataset (\fig\ref{fig:distribution_of_smell_in_dataset}). It shows that all the five types of smells discussed occur in the dataset with a considerable frequency where the most frequent smell in our dataset is `Lazy’ with 275 occurrences and the least frequent smell is `Bloated’ with 141 occurrences.  

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Overall Smell Count Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]%[!htb]
  \centering
  %\hspace*{-.7cm}%
  \includegraphics[scale=.19]{new_images/amount_of_mulitsmell_in_dataset.png}

  %\caption{Number of documentation having multi-smells in our dataset.}
  \caption{Smell distribution by \# of documentation units.}

  \label{fig:amount_of_multismell_in_dataset}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Different Smell Count Image 
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.19]{new_images/distribution_of_smell_in_dataset.png}
 % \vspace{-4mm}
  \caption{Distribution of different smells in our dataset.}

  \label{fig:distribution_of_smell_in_dataset}
\vspace{-4mm}
\end{figure}

%\subsection{Correlation }
%\label{subsec:discussion_correlation}
In multi-label learning, the labels might be interdependent and correlated
\cite{label_correlation_paper_1}. We used Phi Coefficients to determine such
interdependencies and correlations between different documentation smells. The
Phi Coefficient is a measure of association between two binary variables
\cite{phi_coefficient_paper}. It ranges from -1 to +1, where ±1 indicates a
perfect positive or negative correlation and 0 indicates no relationship. We
report the Phi Coefficients between each pair of labels in \fig\ref{fig:label_correlation}. We find that there is almost no correlation between
`Fragmented’ and any other smell (except `Lazy’). By definition, the information
of fragmented documentation is scattered in many sections or pages. Hence, it
has little to do with smells like `Bloated’, `Excess Structural Information’, or
`Tangled’. We also observe that there is a weak positive correlation (+0.2 to
+0.4) among the `Bloated’, `Excess Structural Information’, and `Tangled’
smells. One possible reason might be that if a documentation is filled with
complex and unorganized information (Tangled) or unnecessary structural
information (Excess Structural Information), it might be prone to become bloated
as well. On the other hand, `Lazy’ smell has a weak negative correlation (-0.2
to -0.3) with all other groups since these kinds of documentation are often too
small to contain other smells. However, none of these coefficients is high
enough to imply a strong or moderate correlation between any pair of labels.
Hence, all types of smells in our study are more or less unique in nature.

\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
   \hspace*{-.7cm}%
  \includegraphics[scale=.5]{new_images/label_correlation.png}
 % \vspace{-4mm}
  \caption{Correlation between different documentation smells in our benchmark. 
  Red, Blue, and Gray mean positive, negative, and no correlation. Intensity of color indicates the level of correlation.}

  \label{fig:label_correlation}
\vspace{-5mm}
\end{figure}


% %talk about how data is collected, i.e., how we created the dataset for everyone to label for benchmarks. talk briefly about the benchmark creation process
% We collected documentations of over 29K methods belonging to over 4K classes of
% 217 different packages. We extracted these documentations from the online JAVA
% API Documentation
% website\footnote{\url{https://docs.oracle.com/javase/7/docs/api/}} through web
% crawling and text parsing techniques \cite{web_crawl_book_1,web_crawl_book_2}.
% Then we created a benchmark dataset of 1000 labeled documentation. We used this
% dataset to investigate several machine learning methods to automatically detect
% documentation smells. Since a documentation can contain multiple smells at the
% same time, this is a multi-labeled dataset. We produced the benchmark as
% follows. First, all the authors mutually discussed the documentation smells.
% Then, we randomly selected 1000 documentations from a total of 29K that we
% extracted. Then the first two authors labeled the first 50 documentations
% separately. When they finished, they consulted other co-authors and resolved the
% disagreement based on the discussion. Then they continued with the next 50
% documentations and repeat the same process. Their agreement of labeling has been
% recorded using Cohen’s Kappa Coefficient \cite{cohen_kappa_paper} for each
% iteration, i.e., labeling 50 documentations (Table \ref{cohen_kappa_table}).
% After the third iteration, both the authors reached an acceptable level of
% agreement with Cohen’s Kappa Coefficient of $0.83$. Then they prepared a
% guideline for the labeling task which was later presented to 17 
% undergraduate students who labeled the remaining 850
% documentation units.







% 
% \subsection{Distribution of documentation smells in the benchmark}\label{sec:benchmark_details}
% %give two statistics: all the documentation unit you analyzed and the percentage of which was finally considered as smells.
% %then describe how the different documentation smells are prevalent in the benchmark. 
% %We conducted an exploratory analysis of our labeled dataset. 
% We calculated the total amount of smells in our dataset (\fig\ref{fig:amount_of_multismell_in_dataset}). 
% We found that  778 documentations (almost 78\%) of our dataset contain at least one smell. While most (524) of the smelly documentations contain only one type of smell, a small number (19) of documentations show as high as four smells at the same time. We also determined the distribution of different smells in our dataset (\fig\ref{fig:distribution_of_smell_in_dataset}). It shows that all the proposed smells occur in the dataset with a considerable frequency where the most frequent smell in our dataset is `Lazy’ with 275 occurrences, and the least frequent smell is `Bloated’ with 141 occurrences.  
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Overall Smell Count Image 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \begin{figure}[t]%[!htb]
%   \centering
%   %\hspace*{-.7cm}%
%   \includegraphics[scale=.19]{new_images/amount_of_mulitsmell_in_dataset.png}
% 
%   %\caption{Number of documentation having multi-smells in our dataset.}
%   \caption{Number of documentation having different number of smells in our dataset.}
% 
%   \label{fig:amount_of_multismell_in_dataset}
% 
% \end{figure}
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Different Smell Count Image 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \begin{figure}[t]%[!htb]
%   \centering
%   %\vspace{-6mm}
%   %\hspace*{-.7cm}%
%    \includegraphics[scale=.19]{new_images/distribution_of_smell_in_dataset.png}
%  % \vspace{-4mm}
%   \caption{Distribution of different smells in our dataset.}
% 
%   \label{fig:distribution_of_smell_in_dataset}
% %\vspace{-4mm}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%

==> DocBotSANER2021 (Camera Ready)/conclusions.tex <==
\section{Conclusions}
The learning of an API is challenging when the official documentation resources are of low quality. We identify 
five API documentation smells by consulting API documentation literature on API documentation design and presentation issues.  
We present a benchmark of 1,000 API documentation units with five smells in API official documentation. 
Feedback from 21 industrial software developers shows that the smells can negatively impact the productivity of the developers 
during API documentation usage. We
develop a suite of machine learning classifiers to automatically detect the smells. 
The best performing classifier BERT, a deep learning model, achieves F1-scores of 0.75 - 0.97. 
The techniques can help automatically monitor and warn about API documentation quality.


% 
% In this paper, we make the following novel contributions to the state of the art research in software engineering:
% \begin{enumerate}[leftmargin=15pt]
%     \item\bf{Benchmark.} We present a benchmark of 1,000 API documentation units with five smells in API official documentation. 
%     {To the best of our knowledge, this is the first ever such dataset with real-world examples of the five smells}.
%     We present the feedback from 20 industrial software developers on the prevalence and impact of the smells. 
%     {The developers considered the smells as detrimental to the quality of API documentation} and asked for tool support to automatically detect and fix those.
%     \item\bf{Algorithms.} We develop a suite of techniques to automatically detect the five API documentation smells with more 
%     than 80\% precision and recall. The techniques can be used to automatically detect and monitor the prevalence of the five smells in API official documentation. {To the best of our knowledge, ours are the first techniques developed to detect the five API documentation smells}.
% \end{enumerate}


==> DocBotSANER2021 (Camera Ready)/discussions.tex <==
\section{Discussions}\label{sec:discussions}
\nd\bf{Implications of Findings.} Thanks to the significant research efforts to understand API documentation problems using 
empirical and user studies, we now know with empirical evidence that the quality of API official documentation is a concern both for open source and 
industrial APIs~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Garousi-UsageUsefulnessSoftwareDoc-IST2015,Forward-RelevanceSoftwareDocumentationTools-DocEng2002}.  
The five API documentation smells we studied in this paper are 
frequently referred to as documentation presentation/design problems in the literature~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019}. 
Our comprehensive benchmark of 1,000 API official documentation 
units has 778 units each exhibiting one or more of the smells. The validity of the smells by professional software developers 
proves that this benchmark can be used to foster a new area of research in software engineering on the automatic detection 
of API documentation quality - which is now an absolute must due to the growing importance of APIs and software in our daily lives~\cite{Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Ponzanelli-PrompterRecommender-EMSE2014}. 
The superior performance of our machine learning classifiers, in particular the deep learning model BERT, offers promise that we can now use 
such tools to automatically monitor and warn about API documentation quality in real-time.  
Software companies and open source community can leverage our developed model to analyze the quality of their API documentation. 
Software developers could save time by focusing on good quality API documentation instead of the bad ones as detected by our model.
Based on such real-time feedback, tools 
can be developed to improve the documentation quality by fixing the smells. Indeed, when we asked our survey participants (\sec\ref{sec:survey}) whether 
the five smells need to be fixed, more than 90\% responded with a `Yes', 9.5\% with a `Maybe', 0\% with a `No' (see \fig\ref{fig:smell-fix}).
%\anindya{We may write how such a detection tool may help sponsor of the documentation improve the quality of their documentation. Also, it would save time of the developers who can use the APIs quickly and conveniently.}

% The 
% While the documentation smells do not necessarily make an API documentation
% incorrect, they can hinder the productivity of the developers, according to the
% survey response. Therefore, in this work, we focus on defining the catalog for
% the documentation smells. We show that these documentation smells are prevalent
% in Java official API documentation and by leveraging ML algorithms, we can
% detect them from the documentation texts. The catalog presented in this work can
% be extended to point out the documentation smells more accurately. Moreover, the
% documentation codes can be taken into account along with the documentation texts
% to find out how the detection of the documentation smells can vary depending on
% the documentation codes. The ultimate objective of this research requires manual
% curation of the defected documentations in order to build an automated system
% for correcting the documentation smells.
\begin{figure}[t]
	\centering\begin{tikzpicture}[scale=0.25]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0,
        rotate = -15,
        color={black!10, black!0},
        ]
        {
            9.5/9.5\% Maybe,
            90.5/\bf{90.5\% Yes}\\ smells should be\\ fixed in API\\ documentation
        }
    \end{tikzpicture}
	\caption{Survey responses on whether the five documentation smells should be fixed to improve API documentation quality.}
	\vspace{-5mm}
	\label{fig:smell-fix}
\end{figure}

\nd\bf{Threats to Validity.}  \it{Internal validity} threats relate to authors' bias 
while conducting the analysis. We mitigated the bias in our benchmark creation process by taking agreement 
from 17 coders and co-authors and by consulting API documentation literature. The machine learning models 
are trained, tested, and reported using standard practices. There was no common data between the training and test set. 
\it{Construct validity} threats relate to the difficulty in finding
data to create our catalog of smells. Our benchmark 
creation process was exhaustive, as we processed more than 29K unit examples from official documentation.  
\it{External validity} threats relate to the
generalizability of our findings. We mitigated this threat by corroborating the five smells in our study 
with findings from state-of-the-art research in API documentation presentation and design problems. 
Our analysis focused on the validation and detection of five API documentation smells. Similar to code smell literature, 
additional documentation smells can be added into our catalog as we continue to research on this area.



==> DocBotSANER2021 (Camera Ready)/introduction.tex <==
% %------------------------------------------
\section{Introduction}\label{sec:introduction}
% %------------------------------------------
APIs (Application Programming Interfaces) are interfaces to reusable software
libraries and frameworks. Proper learning of APIs is paramount to support modern day rapid software
development. To support this, APIs typically are supported by official
documentation. An API documentation is a product itself, which warrants the
creation and maintenance principles similar to any existing software product. A
good documentation can facilitate the proper usage of an API, while a bad
documentation can severely harm its
adoption~\cite{Robillard-APIsHardtoLearn-IEEESoftware2009a,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Aghajani-SoftwareDocPractitioner-ICSE2020}. 
%Indeed, API official documentation 
%is often found to be incomplete, incorrect and not usable - problems that can 
%prove as blockers to reuse API features~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a}. 
 
A significant body of API documentation research has focused on studying API documentation problems based on surveys and interviews of software 
developers~\cite{Robillard-APIsHardtoLearn-IEEESoftware2009a,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Aghajani-SoftwareDocPractitioner-ICSE2020,Cai-FrameworkDocumentation-PhDThesis2000,Carroll-MinimalManual-JournalHCI1987a,
Rossen-SmallTalkMinimalistInstruction-CHI1990a,Meij-AssessmentMinimalistApproachDocumentation-SIGDOC1992,Zhia-CostBenefitSoftwareDoc-JSS2015,Garousi-UsageUsefulnessSoftwareDoc-IST2015,Forward-RelevanceSoftwareDocumentationTools-DocEng2002}. 
Broadly, API documentation problems are divided into two types, what (i.e., what is documented) and 
how (i.e., how it is documented)~\cite{Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Uddin-HowAPIDocumentationFails-IEEESW2015}. 
Tools and techniques are developed to address the `what' problems in API documentation, such as 
detection of code comment inconsistency~\cite{rabbi2020detecting,Wen-CodeCommentInconsistencyEmpirical-ICPC2019,Tan-tCommentCodeCommentInconsistency-ICSTVV2012,Zhou-DocumentationCodeToDetectDirectiveDefects-ICSE2017}, 
natural language summary generation of source code~\cite{McBurney-DocumentationSourceCodeSummarization-ICPC2014,Sridhara-SummaryCommentsJavaClasses-ASE2010,Haiduc:Summarization,Moreno-NLPJavaClasses-ICPC2013}, 
adding description of API methods by consulting external resources (e.g., online forums)~\cite{Aghajani-AndroidDocumentation-TSE2019}, 
detecting obsolete API documentation by comparing API version~\cite{Dagenais-DeveloperLearningResources-PhDThesis2012,Dagenais-TraceabilityLinksRecommendDocumentationEvolution-TSE2014},  
and complementing official documentation by incorporating insights and code examples from developer forums~\cite{Treude-APIInsight-ICSE2016,Subramanian-LiveAPIDocumentation-ICSE2014}. 
In contrast, 
not much research has focused on the automatic detection of `how' 
problems, e.g., bad design in API documentation that 
can make the reuse of API features difficult due to lack of usability~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}.
Recently, Treude et al.~\cite{Treude-DocumentationQuality-FSE2020} find that not all API documentation units are equally readable. This finding reinforces 
the needs to automatically detect API documentation presentation issues as `documentation smells', as previously highlighted 
by Aghajani et al.~\cite{Aghajani-SoftwareDocPractitioner-ICSE2020}.
% : \emt{In the case of superfluous content, a compelling next step
% would be to qualitatively study this type of content to
% develop techniques for its automatic detection (similarly
% to the work in code smell detection, with a combination of
% empirical studies~\cite{Tufano-CodeSmellWhenandWhy-TSE2017} and detection techniques~\cite{Moha-DecorCodeDesignSmell-TSE2010}).} 
Unfortunately, we are not
aware of any research on the automatic detection of such API documentation smells.

\begin{figure}[t]
\centering
	\centering
   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
   	\includegraphics[scale=.7]{images/workflow_mod2}
   	\caption{The three major phases used in this study.}
   	 \label{fig:MethodologyOverall}
\vspace{-5mm}
\end{figure}
As a first step towards developing techniques to detect smells in API documentation, 
in this paper, we follow three phases (see \fig\ref{fig:MethodologyOverall}). First, we identify five API documentation 
smells by consulting API documentation literature~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019}  (\sec\ref{sec:benchmark}). 
Four of the smells (bloated, fragmented and tangled description of API documentation unit, and excess structural info in the description) are reported 
as presentation problems by Uddin and Robillard~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 
The other smell is called `Lazy documentation' and it 
refers to inadequate description of an API documentation 
unit (e.g., no explanation of method parameters). Such incomplete documentation is reported  
in literature~\cite{Aghajani-SoftwareDocIssueUnveiled-ICSE2019} and in online discussions. 
We exhaustively explore official API documentation to find the occurrences of the five smells. The focus  
was to develop a benchmark of \it{smelly} API documentation units. A total of 19 human coders 
participated in this exercise. This phase resulted in a benchmark of 1,000 API documentation units, where 778 units have at least one of the five smells.
{To the best of our knowledge, this is the first benchmark with real-world examples of the five documentation smells.}

\begin{figure}[t]
	\centering\begin{tikzpicture}[scale=0.35]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0,
        rotate = -10,
        color={black!10, black!0},
        ]
        {
            4.8/4.8\% Maybe,
            95.2/\bf{95.2\% Yes}\\ documentation\\ smells hinder\\developer producivity
        }
    \end{tikzpicture}
	\caption{Survey responses from professional developers on whether the presence of the smells in API documentation hinders productivity.}
	\vspace{-5mm}
	\label{fig:smell-productivity}
\end{figure}



In the second phase (\sec\ref{sec:survey}), we conducted a survey of 21 professional software developers to validate our catalog of API documentation smells. 
All the participants reported that they 
frequently encounter the five API documentation smells. More than 95\% of the 
participants (20 out of 21) reported that the presence of the five smells in API documentation negatively impacts their productivity (see \fig\ref{fig:smell-productivity}). 
The participants asked for tool support to automatically detect and fix the smells in API official documentation. These findings 
corroborate previous research 
that design and presentation issues in API documentation can hinder API usage~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocPractitioner-ICSE2020}.
In the third phase (\sec\ref{sec:model}), we investigate a suite of rule-based, shallow and deep machine learning models using the benchmark to investigate 
the feasbility of automatically detecting the five smells. The best performing classifer BERT, a deep learning model, achieves F1-scores of 0.75 - 0.97.
{To the best of our knowledge, ours are the first techniques to automatically detect the five API documentation smells}.
{The machine learning models can be used to monitor and warn about API documentation 
quality by automatically detecting the smells in real-time with high accuracy.}

\nd\bf{Replication Package} with benchmark, code, and survey is shared at \url{https://github.com/disa-lab/SANER2021-DocSmell}
% In phase 3, we investigate rule-based, shallow, and deep learning techniques to automatically detect the documentation smells. We answer 
% three research questions.
% 
% \nd\bf{RQ3. How accurate are rule-based classifiers to automatically detect the documentation smells?}
% 
% \nd\bf{RQ4. Can the shallow machine learning models outperform the rule-based classifiers?}
% 
% \nd\bf{RQ5. Can the deep machine learning models outperform the shallow learning models?}

%  
% \begin{enumerate}[label=RQ\arabic{*}., leftmargin=25pt]
%   \item 
%   \item How do software developers perceive of the impact of the detected documentation smells?
%   \item How accurate are rule-based classifiers to automatically detect the documentation smells?
%   \item Can the shallow machine learning models outperform the rule-based classifiers?
%   \item Can the deep machine learning models outperform the shallow learning models?
%   %\item Can the detection of one documentation smell support the detection another smell?
% \end{enumerate}



==> DocBotSANER2021 (Camera Ready)/method.tex <==
\section{Methodology}
\begin{figure*}[t]
\centering
	\centering
   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
   	\includegraphics[scale=.85]{images/workflow_mod3}
   	\caption{The five major steps used in this study}
   	 \label{fig:MethodologyOverall}
\vspace{-5mm}
\end{figure*}
While research is devoted to understand code and design smells, we are aware of no previous research on API documentation smells.
Similar to code and design smells that do not directly introduce a defect or a bug into a software system, documentation smells refer to
presentation issues that do not make a documentation incorrect, rather they hinder its proper usage due to the lack of quality in the design 
and presentation of the documented contents. As such, we studied extensively the API documentation literature that reported issues related to 
API documentation presentation and usability~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019}.  
For example, the most recent paper on this topic was by Aghajani et al.~\cite{Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Aghajani-SoftwareDocPractitioner-ICSE2020}, who 
divided the `how' problems in API documentation into four categories: maintainability (e.g., lenghty files), readability (e.g., clarity), 
usability (e.g., information organization), and usefulness (e.g., content not useful in practice). Previously, Uddin and Robillard~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015} 
studied 10 common problems in API documentation by surveying 323 IBM developers. They observed four common presentation problems: bloated (i.e., too long description), 
tangled (complicated documentation), fragmented (i.e., scattered description), and excess structural info (i.e., content not useful in practice). 
Given that the four problems appeared in both studies, we included each as a documentation smell in our study. In addition, we added lack of 
proper description of an API method as a type of `lazy' smell in the documentation, because incomplete documentation problems are 
discussed in both papers~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocPractitioner-ICSE2020} as well as in online developer discussions. 

Once we decided on the five smells, in the 

That this catalog of five smells provides a good starting point to investigate the focus of this paper, i.e., determining the feasbility of automatically detecting 
the smells using automated techniques. To investigate the techniques, we created our benchmark as follows. 


==> DocBotSANER2021 (Camera Ready)/related-work.tex <==
%------------------------------------------
\section{Related Work}\label{sec:related-work}
%------------------------------------------
Related work is divided into \bf{studies} on understanding (1) documentation problems and (2) how developers learn APIs using documentation, and developing 
\bf{techniques} (3) to detect errors in documentation and (4) to create documentation.

\nd\bf{Studies.} Research shows that traditional Javadoc-type approaches to 
API official documentation are less useful than example-based documentation (e.g., minimal manual~\cite{Carroll-MinimalManual-JournalHCI1987a})~\cite{Shull-InvestigatingReadingTechniquesForOOFramework-TSE2000}
Both code examples and textual description are required for better quality API documentation~\cite{Forward-RelevanceSoftwareDocumentationTools-DocEng2002,DeSouza-DocumentationEssentialForSoftwareMaintenance-SIGDOC2005,Nykaza-ProgrammersNeedsAssessmentSDKDoc-SIGDOC2002}. 
Depending of the types of API documentation, reability and understandability of the documentation can vary~\cite{Treude-DocumentationQuality-FSE2020}. 
Broadly, problems in API official documentation can be about `what' contents are documented and `how' the contents are presented~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Robillard-APIsHardtoLearn-IEEESoftware2009a,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Aghajani-SoftwareDocPractitioner-ICSE2020}. 
Literature in API documentation quality discussed four desired attributes of API documentation: 
completeness, consistency, usability and accessibility \cite{Zhia-CostBenefitSoftwareDoc-JSS2015,Treude-DocumentationQuality-FSE2020}. 
Several studies show that external informal resources can be consulted to improve API official 
documentation~\cite{Yang-QueryToUsableCode-MSR2016,Kavaler-APIsUsedinAndroidMarket-SOCINFO2013,Wang-APIsUsageObstacles-MSR2013,Sunshine-APIProtocolUsability-ICPC2015,Parnin-MeasuringAPIDocumentationWeb-Web2SE2011,Delfim-RedocummentingAPIsCrowdKnowledge-JournalBrazilian2016,Jiau-FacingInequalityCrowdSourcedDocumentation-SENOTE2012}
% The recent focus on API documentation creation from Stack Overflow and online contents is motivated by previous research findings on analyzing the 
% feasibility of Stack Overflow to support API documentation and program comprehension. Parnin and Treude~\cite{Parnin-MeasuringAPIDocumentationWeb-Web2SE2011} 
% analyzed to what extent the methods of an API (jQuery) are documented on the Web. They analyzed 
% 1730 search results and find that 87.9\% of the methods are mainly covered in online blogs and tutorials. Jiau and Yang~\cite{Jiau-FacingInequalityCrowdSourcedDocumentation-SENOTE2012}
% find that API classes with with lower documentation can be covered by another class with more documentation in Stack Overflow, where both are found under same inheritance.  
% Delfim et al.~\cite{Delfim-RedocummentingAPIsCrowdKnowledge-JournalBrazilian2016} find that developers in Stack Overflow provide more content for debugging tasks then for how-to-do tasks.
% Sunshine et al.~\cite{Sunshine-APIProtocolUsability-ICPC2015}  find that 
% developers spent significant time in online forums to seek information about API protocol usage. 
% Studies found code examples from different 
% programming languages can have different usability factors in Stack Overflow~\cite{Yang-QueryToUsableCode-MSR2016}, 
% some Android API classes in the shared code can be more challenging to use than other~\cite{Wang-APIsUsageObstacles-MSR2013}, 
% but there is sub-linear relationship between the Android class popularity in Android apps 
% and the requests for their documentation in Stack Overflow~\cite{Kavaler-APIsUsedinAndroidMarket-SOCINFO2013}. The encouraging documentation coverage in the Web, 
% in participate in Stack Overflow, have motivated us to produce our API documentation from Stack Overflow. 
% Zhang et al.~\cite{Zhang-ReadingAnswerSONotEnough-TSE2019} find that majority of comments posted in Stack Overflow are informative and thus they can enhance the quality of their associated 
% answers. They propose to include comments into knowledge seeking and documentation resources, which traditionally have been only using accepted answers from Stack Overflow.
% Following suggestions from Zhang et al.~\cite{Zhang-ReadingAnswerSONotEnough-TSE2019},  
% we analyze both answers and comments to code examples while producing our API documentation.

The five documentation smells studied in this paper are taken from five commonly discussed API 
documentation design and presentation issues in literature~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocPractitioner-ICSE2020}. 
In contrast to the above papers that aim to understand API documentation problems, we focus on the development of techniques to automatically detect documentation smells.  

\nd\bf{Techniques.} Tools and techniques are proposed to automatically add code examples and insights from external resources (e.g., online forums) into 
API official documentation~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Treude-APIInsight-ICSE2016,Aghajani-AndroidDocumentation-TSE2019}. Topic modeling 
is used to develop code books and to detect deficient documentation~\cite{Souza-CookbookAPI-BSSE2014,Souza-BootstrapAPICodeBookSO-IST2019,Campbell-DeficientDocumentationDetection-MSR2013}. 
API official documentation and online forum data are analyzed together to recommend fixes API misuse scenarios~\cite{Ren-DemystifyOfficialAPIUsageDirectivesWithCorwdExample-ICSE2020}.  
The documentation of an API method can become obsolete/inconsistent due to evolution in source code~\cite{Wen-CodeCommentInconsistencyEmpirical-ICPC2019,Dagenais-DeveloperLearningResources-PhDThesis2012}. 
Several techniques are proposed to automatically detect code comment inconsistency~\cite{rabbi2020detecting,Tan-tCommentCodeCommentInconsistency-ICSTVV2012,Zhou-DocumentationCodeToDetectDirectiveDefects-ICSE2017}. 
A large body of research is devoted to automatically produce natural lanugage summary description of source code method~\cite{McBurney-DocumentationSourceCodeSummarization-ICPC2014,Sridhara-SummaryCommentsJavaClasses-ASE2010,Haiduc:Summarization,Moreno-NLPJavaClasses-ICPC2013}. 

Unlike previous research, we focus on the detection of five API documentation smells that do not make a 
documentation inconsistent/incorrect, but nevertheless make the learning of the documentation difficult due to the underlying design/presentation issues. 
We advance state-of-the-art research on API documentation quality analysis by offering a benchmark of real-world examples of five documentation smells 
and a suite of techniques to automatically detect the smells. 
% \subsection{Studies on API Documentation Problems}
% APIs (Application Programming Interfaces) are interfaces to reusable software libraries and frameworks. The proper learning of APIs is paramount to support modern day rapid software development. To achieve this goal, APIs typically are supported by official documentation. An API documentation is a product itself, which warrants the creation and maintenance principles similar to any existing software product. A good documentation can facilitate the proper usage of an API, while a bad documentation can severely harm its adoption~\cite{Robillard-APIsHardtoLearn-IEEESoftware2009a}.
% Unfortunately, research shows that API official documentation can be often incomplete, incorrect, and outdated~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 
% TODO: expand
% \subsection{How developers learn to select and use APIs}
% 
% 
% Robillard and DeLine~\cite{Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a} 
% conducted a survey and a series of qualitative interviews of software developers
% at Microsoft to understand how developers learn APIs. The study identified
% that the most severe obstacles developers faced while learning new APIs were
% related to the official documentation of the APIs. With API
% documentation, the developers cited the lack of code examples and the absence of task-oriented
% description of the API usage as some major blockers to use
% APIs.  
% 
% 
% Carroll et al.~\cite{Carroll-MinimalManual-JournalHCI1987a} observed developers
% while using traditional documentation to learn an API (e.g., Javadoc, manual).
% They found that the learning of the developers was often interrupted by
% their self-initiated problem-solving tasks that they
% undertook during their navigation of the documentation. During such unsupervised
% exploration, they observed that developers ignored groups and entire sections of
% a documentation that they deemed not necessary for their development task in
% hand. Unsurprisingly, such unsupervised exploration often led to mistakes. They
% conjectured that traditional API documentation is not designed to support such
% active way of developers' learning. To support developers' learning of APIs from
% documentation, they designed a new type of API documentation, called as the
% \it{minimal manual}, that is task-oriented and that helps the users resolve
% errors~\cite{Cai-FrameworkDocumentation-PhDThesis2000,Carroll-MinimalManual-JournalHCI1987a,
% Rossen-SmallTalkMinimalistInstruction-CHI1990a,Meij-AssessmentMinimalistApproachDocumentation-SIGDOC1992}.
% 
% Shull et al.~\cite{Shull-InvestigatingReadingTechniquesForOOFramework-TSE2000}
% conducted a study of 43 participants to compare the effectiveness of
% example-based documentation with hierarchy-based documentation. The
% example-based documentation contained example applications that were found within the
% framework that the participants used. The hierarchy-based documentation is
% similar to the Javadocs, where the classes were presented. Participants were
% specifically taught on how to use the hierarchy-based documentation. However, they abandoned
% it in favor of the example applications based documentation, because it took
% them longer to start writing application using the hierarchy-based
% documentation.
% 
% Forward and
% Lethbridge~\cite{Forward-RelevanceSoftwareDocumentationTools-DocEng2002}
% conducted a survey of 48 software developers and managers. The goal was to
% understand the perceived importance of software documentation and the required
% tools and techniques to maintain those. The participants considered the content
% (information and use of examples) and organization (index, sections) of the
% documents as the most important, as well as the recency and availability of
% such information. 
% 
% De Souza et
% al.~\cite{DeSouza-DocumentationEssentialForSoftwareMaintenance-SIGDOC2005}
% studied the relative importance of the various documentation artifacts using
% two surveys of software developers.
% They identified 24 artifacts based on the responses from software developers,
% such as, source code, comments, data model, test plan, gloassary, etc. More than 92\%
% of the participants considered source code to be most important in the
% documentation, followed by comments (78.2\%) and logical data model (74.6\%).
% 
% Nykaza et al.~\cite{Nykaza-ProgrammersNeedsAssessmentSDKDoc-SIGDOC2002} assessed
% the needs on the desired and required content of API documentation in a software
% organization. They found similar needs among junior programmers with extensive
% knowledge of a domain and the experienced programmers with no knowledge of the
% domain. The common needs among them pertained to the availability of code
% examples that are easy to understand and used for a given task. The developers
% also preferred self-contained sections in API documentation, as opposed 
% to a manual that is fragmented and long, and needed to be completed from the
% start to finish before writing the code. 
% 
% The advent of cloud-based software development has popularized the adoption
% of Web APIs, such as, the Google Map APIs, API mashups in the ProgrammableWeb, and
% so on. Tian et al.~\cite{Tian-ExploratoryStudyWebApi-EASE2017} conducted an
% exploratory study to learn about the features offered by the Web APIs 
% via the ProgrammableWeb portal and the type of contents supported in the
% documentation of those APIs. They observed that such Web APIs offer diverse
% development scenarios, e.g., text mining, business analysis, and so on. They
% found that the documentation of the APIs offer insights into different
% knowledge types, e.g., the underlying intent of the API features, the
% step-by-step guides, and so on.
% 
% During our user studies (in \sec\ref{sec:opinercode-evaluation-effectiveness})
% involving both professional software developers and students, we found that the
% developers were more productive while using the usage summaries in Opiner. In a
% way, the summaries in Opiner are task-based in that they correspond to
% specific development problems the developers discussed in Stack Overflow. We can
% corroborate to the findings of Forward and
% Lethbridge~\cite{Forward-RelevanceSoftwareDocumentationTools-DocEng2002} and De
% Souza et
% al.~\cite{DeSouza-DocumentationEssentialForSoftwareMaintenance-SIGDOC2005} that
% developers prefer the quality of the contents in the API documentation the most,
% in multiple observations.
% \subsection{Automated API Documentation Efforts}
% The inference of API usage patterns and properties by mining software repositores (e.g., version history of client software) has been 
% an active research area for over a decade. Dynamic analysis is used on the execution traces to detect usage
% patterns~\cite{Lo-MiningHierarchicalScenarioBasedSpec-ASE2009,Lo-MiningIterativePatterns-SIGKDD2007,Fahland-MiningBranchingTimeScenarios-ASE2013,Safyallah-PatternMiningDynamicAnalysis-ICPC2006}.
% The techniques instrument software and collect execution traces by running the
% software for relevant task scenarios. Static analysis is used on the version control
% data of software to find API usage
% concepts~\cite{Uddin-TemporalApiUsage-ASE2011,Uddin-TemporalApiUsage-ICSE2012,Robillard-AutomaticSuggestionProgramNavigation-FSE2005,Robillard-RecommendChangeClusters-JournalSoftwareMaintain2010a,Robillard-RepresentingConcern-PhDThesis2003}.
% Unlike above research, we mine API usage scenarios from developer forum, Stack Overflow.  
% 
% The automated mining of crowd-sourced knowledge from developer forums to support API documentation has broadly focused on two areas in recent years:
% \begin{inparaenum}
% \item Creation of API documentation and usage patterns from crowd-sourced knowledge, and 
% \item Assessing the quality and feasibility of crowd-sourced developer knowledge.
% \end{inparaenum} 
%  
% % 
% % To offer a point of reference of our analysis of related work, we review 
% % the research papers listed in the Stack Exchange question `Academic Papers Using Stack 
% % Exchange Data'~\cite{website:sopaper} and whose titles contain the keywords 
% % (`documentation' and/or `API')~\cite{Wang-APIsUsageObstacles-MSR2013,
% % Kavaler-APIsUsedinAndroidMarket-SOCINFO2013,Souza-CookbookAPI-BSSE2014,
% % Sunshine-APIProtocolUsability-ICPC2015,
% % Mastrangelo-JavaUnsafeAPIs-OOPSLA2015,
% % YeDeheng-ExtractAPIMentions-ICSME2016,Campos-SearchSORecommend-JSS2016,
% % Campos-SearchSOPostAPIBug-CASCON2016,
% % Azad-GenerateAPICallrules-TOSEM2017,
% % Ahsanuzzaman-ClassifySOPost-SANER2018,Wang2013Detecting,
% % Dagenais-DeveloperDocumentation-FSE2010a,
% % Parnin-MeasuringAPIDocumentationWeb-Web2SE2011,
% % Parnin2012,Jiau-FacingInequalityCrowdSourcedDocumentation-SENOTE2012,
% % Campbell-DeficientDocumentationDetection-MSR2013,
% % Treude-DocumentationInsightsSO-ICSE2016,
% % Delfim-RedocummentingAPIsCrowdKnowledge-JournalBrazilian2016,
% % LiXing-LeveragingOfficialContentSoftwareDocumentation-TSC2018,
% % LiSun-LearningToAnswerProgrammingQuestions-JIS2018}.    
% % Existing research on API documentation efforts using crowd-sourced knowledge have focused on the following areas: 
% % \begin{enumerate}[leftmargin=10pt]
% % \item Producing API Documentation and Usage Patterns,
% % %\item Traceability recovery of API elements in forum posts,
% % \item Assessing the feasibility of forum contents for API documentation and design needs, and
% % %\item Answering to API-related questions.
% % %\item Categorizing forum contents for information discovery, and
% % \end{enumerate} 
%  
% 
% 
% 
% 
% 
% 
% %\subsubsection{Producing API Documentation and Usage Patterns.} 
% Javadocs are annotated by Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014} to add code examples to the official documentation 
% of an API type (e.g., class) from Stack Overflow and by API Insight~\cite{Treude-APIInsight-ICSE2016} to add important textual insights 
% about the API type. Unlike Baker and API Insight, we produce stand-alone API documentation by proposing two novel algorithms: Statistical and Concept-Based. 
% API sequence (e.g., one after another or together) 
% calls are mined by Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016} from GitHub code repositories and by Azad et al.~\cite{Azad-GenerateAPICallrules-TOSEM2017} 
% on Android code base and Stack Overflow code examples. We do not produce API sequence calls in our API documentation. Instead, in our concept-based 
% documentation we find API usage scenarios that are conceptually relevant to each other. Li et al.~\cite{LiXing-LeveragingOfficialContentSoftwareDocumentation-TSC2018} 
% propose CnCxL2R, a software documentation recommendation 
% engine by incorporating the content of the official documentation with social context from Stack Overflow. 
% Souza et al.~\cite{Souza-CookbookAPI-BSSE2014,Souza-BootstrapAPICodeBookSO-IST2019} propose a semi-automatic approach based 
% on topic modeling to build cookbooks for APIs by organizing 
% knowledge available in Stack Overflow. Topic modeling was also applied by Campbell et al.~\cite{Campbell-DeficientDocumentationDetection-MSR2013} 
% on a combined dataset of Stack Overflow, and PHP and Python official documentation to determine missing topic coverage in the official documentation. 
% Ren et al.~\cite{Ren-DemystifyOfficialAPIUsageDirectivesWithCorwdExample-ICSE2020} 
% develop a text mining approach to discover API misuse scenarios in Stack Overflow. 
% They extract erroneous code examples, patches, related and confusing APIs from the misuse scenarios and construct demystification reports. 
% The reports can be 
% used to help developers understand the official API usage directives. 
% Unlike the above work, we also 
% consider reviews about code examples while producing the documentation. In our previous surveys of 178 software 
% developers, we found that developers consider the combination of code examples and reviews about the examples as a form of API documentation and they 
% value such documentation over official documentation.
% 
% % 
% To produce API documentation from crowd-sourced forum, we first need to link code examples to APIs.
% A number of techniques automatically infer code terms (e.g., API method, class)
% in textual contents and code examples of forum posts (see \cite{Dagenais-RecoDocPaper-ICSE2012a},
% \cite{Subramanian-LiveAPIDocumentation-ICSE2014}, \cite{Rigby-CodeElementInformalDocument-ICSE2013}, \cite{YeDeheng-ExtractAPIMentions-ICSME2016},
% \cite{Phan-StatisticalLearningFQNForums-ICSE2018},
% and \cite{Ma-APINERSODeepLearning-TSE2019}).
% Unlike above techniques, we associate a code example to an
% API mentioned in the textual contents of the forum post, about which the code example is provided. Therefore, we do not link
% \it{all} the different APIs whose classes are used in the code example or all different API/code elements that are mentioned in the textual contents.
% In our previously published paper~\cite{Uddin-MiningAPIUsageScenarios-IST2020}, we showed that this approach is better suited to produce
% task-centric~\cite{Carroll-MinimalManual-JournalHCI1987a,DeSouza-DocumentationEssentialForSoftwareMaintenance-SIGDOC2005}
% API documentation from Stack Overflow, where an API is of particular focus to complete a task. 
% %Chen et al.~\cite{Chen-SEthesaurusSO-TSE2015} propose a technique to build SE (Software Engineering)-specific thesaurus by crawling Stack Overflow. 
% %The thesaurus can be used to further improve the detection of API mentions and technological 
% %terms during the mining of API discussions and code example, including the mining techniques that we used in this paper.
% 
% % 
% % 
% % The GitHub code repositories are mined by Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016} 
% % produce sequence of API elements to complete a coding task. 
% % Unlike Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016}, we 
% % mine and summarize API usage scenarios involving the usage of API elements to produce API documentation. 
% % Unlike Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016}, we associate reactions 
% % to offer insights into code examples.  
% % 
% % Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014} proposes live API documentation by automatically
% % annotating Javadocs of API classes by code examples from accepted answers in Stack Overflow where the
% % API classes are used. Unlike Baker, we do not augment Javadoc. Instead, we produce the documentation in a stand-alone portal 
% % where the documentation of any API can be viewed based on our two proposed novel algorithms. API insight~\cite{Treude-APIInsight-ICSE2016} annotates Javadocs of API
% % types by collecting important insights from the textual contents of forum posts
% % where the types are discussed. Unlike Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014} and 
% % API Insight~\cite{Treude-APIInsight-ICSE2016}, we leverage reviews (i.e., positive and negative opinions) 
% % to inform of the quality of code examples. The GitHub code repositories are mined by Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016} 
% % produce sequence of API elements to complete a coding task. 
% % Unlike Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016}, we 
% % mine and summarize API usage scenarios involving the usage of API elements to produce API documentation. 
% % Unlike Gu et al.~\cite{KimGu-DeepAPILearning-FSE2016}, we associate reactions 
% % to offer insights into code examples.  
% % 
% % 
% % 
% % 
% % Li et al.~\cite{LiXing-LeveragingOfficialContentSoftwareDocumentation-TSC2018} propse CnCxL2R, a software documentation recommendation 
% % engine by incorporating the content of the official documentation with social context from Stack Overflow. The recommendation is a learning-to-rank schema. 
% % They evaluate the engine on Java documentation recommendation. 
% % 
% % Azad et al.~\cite{Azad-GenerateAPICallrules-TOSEM2017} cluster co-changing API calls used by 230 Android apps across 12K versions to predict API calls that 
% % individual developers can use. They then apply similar technique by grouping API calls in each positively voted answers in Stack Overflow. The first technique 
% % achieves 75\% precision and 22\% recall. The Stack Overflow-based techniques achieves 66\% precision and 13\% recall.  
% % 
% % 
% % Campbell et al.~\cite{Campbell-DeficientDocumentationDetection-MSR2013} combined questions from Stack Overflow and documentation from PHP and Python 
% % projects and apply topic modeling on the combined datasets to determine any topics which are inadequately covered in the project documentation. They found topics 
% % in need of tutorial documentation. 
%  
% % Ren et al.~\cite{Ren-DemystifyOfficialAPIUsageDirectivesWithCorwdExample-ICSE2020} develop a text minin approach to discover API misuse scenarios in Stack Overflow. 
% % The extract erroneous code examples, patches, related and confusing APIs from the misuse scenarios and construct demystification reports. The reports can be 
% % used to help developers understand the official API usage directives. 
% 
% 
% 
% % Souza et al.~\cite{Souza-CookbookAPI-BSSE2014,Souza-BootstrapAPICodeBookSO-IST2019} propose a semi-authomatic approach to build cookbooks for APIs by organizing 
% % knowledge available in Stack Overflow. 
% % The approach first identifies threads with How to questions in Stack Overflow for a given API (e.g., SWT). Topic modeling is applied on the threads to determine individual chapters 
% % of a codebook. They also define desired properties that such crowd codebooks must meet. They evaluate the desired properties against human subjects.  
% 
% 
% %\cite{Li-LeverageOfficialContentToRecommendDocSO-TSC2018}
% 
% 
% %\subsection{Answering to API-related questions}
% %\subsection{Mining API Usage Patterns}
% %\nd\bf{Mining Usage Patterns from Execution Traces.} 
% 
% 
% % \subsubsection{Assessing Quality and Documentation Feasibility of Forum Contents} 
% % The recent focus on API documentation creation from Stack Overflow and online contents is motivated by previous research findings on analyzing the 
% % feasibility of Stack Overflow to support API documentation and program comprehension. Parnin and Treude~\cite{Parnin-MeasuringAPIDocumentationWeb-Web2SE2011} 
% % analyzed to what extent the methods of an API (jQuery) are documented on the Web. They analyzed 
% % 1730 search results and find that 87.9\% of the methods are mainly covered in online blogs and tutorials. Jiau and Yang~\cite{Jiau-FacingInequalityCrowdSourcedDocumentation-SENOTE2012}
% % find that API classes with with lower documentation can be covered by another class with more documentation in Stack Overflow, where both are found under same inheritance.  
% % Delfim et al.~\cite{Delfim-RedocummentingAPIsCrowdKnowledge-JournalBrazilian2016} find that developers in Stack Overflow provide more content for debugging tasks then for how-to-do tasks.
% % Sunshine et al.~\cite{Sunshine-APIProtocolUsability-ICPC2015}  find that 
% % developers spent significant time in online forums to seek information about API protocol usage. 
% % Studies found code examples from different 
% % programming languages can have different usability factors in Stack Overflow~\cite{Yang-QueryToUsableCode-MSR2016}, 
% % some Android API classes in the shared code can be more challenging to use than other~\cite{Wang-APIsUsageObstacles-MSR2013}, 
% % but there is sub-linear relationship between the Android class popularity in Android apps 
% % and the requests for their documentation in Stack Overflow~\cite{Kavaler-APIsUsedinAndroidMarket-SOCINFO2013}. The encouraging documentation coverage in the Web, 
% % in participate in Stack Overflow, have motivated us to produce our API documentation from Stack Overflow. 
% % Zhang et al.~\cite{Zhang-ReadingAnswerSONotEnough-TSE2019} find that majority of comments posted in Stack Overflow are informative and thus they can enhance the quality of their associated 
% % answers. They propose to include comments into knowledge seeking and documentation resources, which traditionally have been only using accepted answers from Stack Overflow.
% % Following suggestions from Zhang et al.~\cite{Zhang-ReadingAnswerSONotEnough-TSE2019},  
% % we analyze both answers and comments to code examples while producing our API documentation.
% 
% 
%  
% 
% % Yang et al.~\cite{Yang-QueryToUsableCode-MSR2016} analyzed the usability of 3M code snippets in Stack Overflow based on whether 
% % the provided code as-is can be used in a program generation tool. This requires three steps: parsing, compiling and running the source code. 
% % Among they four languages they analyzed, Python and Javascript code snippets are found to have more usable code snippets while Java and C\# are proved to have the 
% % lowest usability rate.   
% % 
% % Wang and Godfrey~\cite{Wang-APIsUsageObstacles-MSR2013} analyze the obstacles of learning iOS and Android APIs. They identify several 
% % challenging APIs classes. For each of those APIs, they collect Stack Overflow posts tagged as the APIs and then apply topic modeling on the 
% % posts to discover repetitive scenarios in which the API usage obstacles could occur. They offer guidelines to API designers to mitigate the obstacles.
% % 
% % Kavaler et al.~\cite{Kavaler-APIsUsedinAndroidMarket-SOCINFO2013} analyze data from Android applications and Stack Overflow together to understand the needs 
% % of software developers. They find 
% % a sub-linear relationship between the class popularity in Android apps and the requests for their documentation in Stack Overfow, i.e., the number of questions in Stack Overflow lags 
% % its total usage in the Android apps. They also find larger classes and more documented classes are associated with more answers. Overall, the 
% % documentation size of an API class has a strong positive relationship with getting first answer in Stack Overflow. That means, users are more inclined to answer the question related to 
% % an API that class that has larger documentation. 
% 
% 
% % Sunshine et al.~\cite{Sunshine-APIProtocolUsability-ICPC2015} analyze Stack Overflow posts to understand the challenges developer face while learning API usage 
% % protocols. They identify a list of distinct protocol specific tasks. They then recruit developers and ask them to complete the tasks in lab settings. They find that 
% % the developers spent significant time to seek information. For the debugging of protocol violations, the developers sought to find help from documentation.
% % 
% % Parnin and Treude~\cite{Parnin-MeasuringAPIDocumentationWeb-Web2SE2011} analyzed to what extent the methods of an API (jQuery) are documented on the Web. They analyzed 
% % 1730 search results and find that 87.9\% of the methods are mainly covered in online blogs and tutorials. However, the efforts are concentrated around a handful of primary developers. 
% % In a subsequent study, Parnin et al.~\cite{Parnin2012} how Stack Overflow faciliate crowd documentation. They examine the Stack Overflow for three popular APIs (Android, GWT and the Java 
% % Programming Language). They collect usage data from Google code search and use Stack Overflow documentation to analyze the coverage, quality, and dynamics of the APIs. 
% % They find that the crowd-documentation is rich with code examples and discussions and it is viewed and used by many developers. 
% % 
% % Jiau and Yang~\cite{Jiau-FacingInequalityCrowdSourcedDocumentation-SENOTE2012} analyze the inequality of documentation in Stack Overflow based on the notion that inequality 
% % may arise when a larger portion of crowd-sourcing resources is allocated to a smaller percentages of topics. They propose to reduce the inequality 
% % based on the analysis of inheritence in Object-Oriented Language, i.e., by leveraging the numerous duplications among classes of an API that belong to the same inheritence 
% % hierarchy. Thus the one with lower documentation can be covered by another class with more documentation, where both are found under same inheritence.  
% % They analyze three APIs (Swing, SWT, and GWT) and found the method effective.
% %  
% % 
% % Zhang et al.~\cite{Zhang-ReadingAnswerSONotEnough-TSE2019} find that majority of comments posted in Stack Overflow are informative and thus they can enhance the quality of their associated 
% % answers. They propose to include comments into knowledge seeking and documentation resources, which traditionally have been only using accepted answers from Stack Overflow.
% % 
% % Delfim et al.~\cite{Delfim-RedocummentingAPIsCrowdKnowledge-JournalBrazilian2016} conduct a study using Stack Overflow data to understand how 
% % crowd can contribute to API documentation in two programming tasks: how to implement a scenario using an API and how to fix bugs regarding the usage of an API. 
% % They find that developers in Stack Overflow provide more content for debugging tasks then for how-to-do tasks.  
% 
% %\subsubsection{Quality Analysis of Crowd-Sourced Development Knoweldge}
% % The encouraging findings on the feasibility and availability of crowd-sourced knowledge have motivated researchers to also 
% % analyze the quality of the shared knowledge. A number of recent research papers~\cite{Zhang-AreCodeExamplesInForumReliable-ICSE2018,Yang-QueryToUsableCode-MSR2016,Terragni-CSNIPPEX-ISSTA2016} 
% % warn against directly copying code from Stack Overflow, because such code can have potential bugs or 
% % misuse patterns~\cite{Zhang-AreCodeExamplesInForumReliable-ICSE2018} and that such code 
% % may not be directly usable (e.g., not compilable)~\cite{Yang-QueryToUsableCode-MSR2016,
% % Terragni-CSNIPPEX-ISSTA2016}. Mondal et al.~\cite{Mondal-SOIssueReproducability-MSR2019} analyze the reproducibility of code example shared in Stack Overflow questions. They find that questions with 
% % reproducible problem in the code example are three times more likely to be answered. 
% % Mastrangelo et al.~\cite{Mastrangelo-JavaUnsafeAPIs-OOPSLA2015} investigate the spread of unsafe Java code that are used as ``backdoors'' in Java runtime to facilitate 
% % high-performance system level code in Java. They analyze 74GB of compiled Java code, spread over 86,479 Java archives. They find that 25\% of the Java archives use such unsafe code.
% % Zhang et al.~\cite{Zhang-ObsoleteAnswerSO-TSE2019} analyze answers with obsolete solutions in Stack Overflow. They find that more than 50\% of those obsolete answers were obsolete even during 
% % the time of their creation. They find that answers to questions related to node.js, ajax, android, and objective-c are more likely to become obsolete. 
% % Tools and techniques are also proposed to detect high quality posts and answers~\cite{Ponzanelli-ImproveLowQualityPostDetect-ICSME2014}.
% % \rev{Recently, Ren et al.~\cite{Ren-DiscoverControversialDiscussions-ASE2019} propose a technique to discover answers that are being criticized in Stack Overflow for having erroneous 
% % solutions. They identify such critique posts as controversial discussions. They then summarize the controversial discussions per problematic answer. 
% % In our current Opiner API documentation framework, we inform developers of problems in the code examples by showing them negative opinions provided 
% % against the code examples in the comments to the answers. The developers in our user studies mentioned that such insights are very useful. The produced 
% % API documentation can be made more useful by highlighting controversial discussions about a code example, by utilizing the techniques from Ren et al.~\cite{Ren-DiscoverControversialDiscussions-ASE2019}.}
% % 
% % Ragkhitwetsagul et al.~\cite{Ragkhitwetsagul-ToxicCodeSO-TSE2018} identify toxic code in Stack Overflow as the code examples that are outdated or that violate original software 
% % license. They conduct a survey of 201 high-reputation Stack Overflow users and find that they rarely check for license violation. 
% % Violation of licenses is a common problem for code examples shared in other platforms, such as Android Ecosystem (see Mlouki et al.~\cite{Mlouki-LicenseViolationAndroid-SANER2016}). 
% % All documented API usage scenarios in Opiner can be further enhanced by the information of license that need to be adopted before the reuse of a code example. This can 
% % help reduce the above license violation problems.
%  
% % to inform developers of potential problems in answers, such as detecting controversies between answers and comments and proposing solutions to fix the 
% % controversies.  
% % 
% % 
% % Given the advance in techniques developed to automatically mine insights from crowd-sourced software 
% % forums, recent research on crowd-sourced API documentation has focused specifically on the analysis of quality 
% % in the shared knowledge. 
% % 
% % 
% % 
% % 
% % 
% % 
% % Ragkhitwetsagul et al.~\cite{Ragkhitwetsagul-ToxicCodeSO-TSE2018} identify toxic code in Stack Overflow as the code examples that are outdated or that violate original software 
% % license. They conduct a survey of 201 high-reputation Stack Overflow answeres and find that 65\% were never notified of such code and they rarely check for license violation. 
% % Violation of licenses is a common problem for code examples shared in other platforms, such as Android Ecosystem (see Mlouki et al.~\cite{Mlouki-LicenseViolationAndroid-SANER2016}).    
% % 
% % We observed both issues during the development of our proposed mining framework. We attempted to 
% % offer solutions to both issues within the context of our goal, i.e., producing task-based documentation. 
% % Therefore, to ensure such code examples can still be included in our task-based documentation, we used a 
% % hybrid code parser that combines Island parsing with ANTLR grammar to parse code examples line by line (see \cite{Uddin-MiningAPIUsageScenarios-IST2020}). 
% 
% 
% % \subsection{Assisting Development Task Completion Using Crowd-Sourced Knowledge}
% % A number of tools are developed to offer context-aware code completion information into the IDE of a developer based on crowd-sourced knowledge. 
% % Zilberstein and Yahav~\cite{Zilberstein-Codota-ONWARD2016} proposed an approach 
% % to leverage code examples from forum posts to support auto code completion features in IDEs.
% % They built Codota, a tool that given a code context from the IDE, 
% % automatically searches forum posts to find most relevant code examples that can be relevant to the code context.
% % Ponzanelli et al.~\cite{Ponzanelli-PrompterRecommender-EMSE2014} developed an
% % Eclipse Plug-in that takes into account the source code in a given file as a
% % context and use that to search Stack Overflow posts to find relevant discussions
% % (i.e., \it{code to relevant information}). Campbell and Treude~\cite{Campbell-NLP2Code-ICSME2017} develop NLP2Code that integrates with a developer's IDE to provide him with 
% % a content assist feature to close the vocabulary gap between the needs of the developer and the code snippet meta data. 
% % While the above tools extend IDEs, Opiner is a stand-alone portal to show 
% % API documentation from Stack Overflow. Unlike the above tools that only use code example/discussions, Opiner use code example and reviews. 
% % 
% % 
% % Developers query for technical contents online. A number of techniques are proposed to provide better results to an input technical query by 
% % leveraging crowd-sourced knowledge.  Campos et al.~\cite{Campos-SearchSOPostAPIBug-CASCON2016} propose an approach to find fixes to API-related bugs bugs by matching code snippet that are being 
% % debugged against related snippets in Stack Overflow. To find the API-related bugs, they used OHLOH code search engine containing potentially buggy API method calls. 
% % Rahman et al.~\cite{Masud-QueryReformulationSO-EMSE2019,Masud-RACK-ICSE2017,Masud-RACK-ICSME2016,Masud-NLP2API-ICSME2018} 
% % propose RACK and NLP2API that suggest a list of relevant API classes for a natural 
% % language query intended for code search. The technique exploits keyword-API associations from Stack Overflow posts to reformulate the queries. 
% % Silva et al.~\cite{Silva-RecommendSolutionTaskUsingSO-ICPC2019} propose a tool CROKAGE (Crowd Knowledge Answer Generator) that 
% % takes as input a natural language query of the description of a programming task and outputs solutions to the task by offering code examples 
% % and explanations. The query is expanded with relevant API classes from Stack Overflow. Li et al.~\cite{LiSun-LearningToAnswerProgrammingQuestions-JIS2018} develop QDLinker, a deep-learning-to-answer framework to answer programming questions with software 
% % documentation. The tool learns from the discussions in Stack Overflow to bridge the semantic gap between the types of questions asked and software documentation. 
% % Based on the learning, the tool can effectively answer a programmer question with links to software documentation. Unlike the above techniques, 
% % all the documentation of an API in Opiner can be searched by simply searching by the API name. 
% % Thus Opiner can be extended with above techniques, so that developers can search Opiner API documentation using 
% % natural language query. In fact, during our surveys, this is also one of the features that developers wished Opiner could have in future extensions.
% % 
% % Recently, bots are developed to assist developers in diverse development tasks by utilizing crowd-sourced knowledge. Xu et al.~\cite{BowenXu-AnswerBot-ASE2017} develop AnswerBot that takes as input a natural language description of a programming task. The tool 
% % finds questions relevant to the query and summarizes the useful answers from those questions. Tian et al.~\cite{YuanTian-APIBot-ASE2017} develop APIBot to answer API questions given API documentation as an input. The Bot is built by adapting SiriusQA, a cross-domain 
% % intelligent personal assistant. The engine achieve a Hit@5 score of 0.706 to answer the questions. Future extensions of the bots can also target the curated API documentation in Opiner.
% % 
% % Finally, contents in Stack Overflow can be better used, if the underlying contexts can be better processed. 
% % Ahsanuzzaman et al.~\cite{Ahsanuzzaman-ClassifySOPost-SANER2018,Ahasanuzzaman-ClassifyIssueSO-EMSE2019} develop machine learning classifier to automatically label Stack Overflow questions 
% % describing an issue or not. Terragni et al.~\cite{Terragni-CSNIPPEX-ISSTA2016} investigate the compilability issues with the code snippets shared in Stack Overflow. They developed CSnippEx 
% % that can automatically convert a shared Java code into a compilable code by resolving external dependencies, import statements and syntax errors. Both of these 
% % techniques can help extend the API documentation in Opiner, e.g., by producing compilable code using CSnippEx.
% 
% 
% % 
% % 
% % 
% % Campos et al.~\cite{Campos-SearchSOPostAPIBug-CASCON2016} propose an approach to find fixes to API-related bugs bugs by matching code snippet that are being 
% % debugged against related snippets in Stack Overflow. To find the API-related bugs, they used OHLOH code search engine containing potentially buggy API method calls. 
% % They find that 66.7\% of those bugs can be fixed using code excerpts fom Stack Overlfow. 
% %  
% % Rahman et al.~\cite{Masud-QueryReformulationSO-EMSE2019,Masud-RACK-ICSE2017,Masud-RACK-ICSME2016} propose RACK, a query reformulation technique that suggests a list of relevant API classes for a natural 
% % language query intended for code search. The technique exploits keyword-API associations from Stack Overflow posts. 
% % 
% % Silva et al.~\cite{Silva-RecommendSolutionTaskUsingSO-ICPC2019} propose a tool CROKAGE (Crowd Knowledge Answer Generator) that 
% % takes as input a natural language query of the description of a programming task and outputs solutions to the task by offering code examples 
% % and explanations. The query is expanded with relevant API classes from Stack Overflow. 
% % 
% % Rahman and Roy~\cite{Masud-NLP2API-ICSME2018} propose NLP2API to reformulate queries using crowd-sourced knowledge and extra-large scale data analytics from Stack Overflow. 
% % 
% % Rahman et al.~\cite{Masud-RecommendInsightfulCommentsSO-SCAM2015} present a technique to mine insightful comments from Stack Overflow. The comments 
% % are useful to better understand the provided code example in the answer post of the comments. 
% % 
% % 
% % Xu et al.~\cite{BowenXu-CrossLanguageRelevantQuestion-EMSE2017} propose cross-language relevant question retrieval (CLRQR) tool to relevant English question fo a given 
% % Chinese question. The motivation is that Chinese developers often cannot effectively search questions in English. 
% % 
% % Xu et al.~\cite{BowenXu-PredictSemanticLinkableKnowledgeInForumsCNN-ASE2016} use deep learning with word embedding to address the problem of vocabulary mismatch between a developer's query 
% % and the actual task description.
% % 
% % Zilberstein and Yahav~\cite{Zilberstein-Codota-ONWARD2016} proposed an approach 
% % to leverage code examples from forum posts to support auto code completion features in IDEs.
% % They built Codota, a tool that given a code context from the IDE, 
% % automatically searches forum posts to find most relevant code examples that can be relevant to the code context.
% % While the focus of both Opiner and Codota remains the same, i.e., assisting developers in their
% % development activities, Opiner differs from Codota as follows:
% % \begin{inparaenum}%[leftmargin=4mm]
% % \item \bf{Documentation Vs. Recommendation.} 
% % Opiner mines and documents API usage
% % scenarios. Codota provides recommendations to assist in code auto completion depending on the
% % code context in a developer IDE.
% % %\item \bf{Documentation Vs. IDE.} Opiner's focus is to offer improvements over developers' usage of formal and informal API documentation, 
% % %by producing automated summaries of usage scenarios from forum posts. Codota is a real-time assistant that aim to facilitate auto code-completion in the developers' IDE.
% % \item \bf{Diversity.} Opiner documentation can assist developers in their coding tasks, and support their diverse development 
% % scenarios, e.g., their selection of an API as well.
% % \end{inparaenum} Unlike Codota, Opiner supports the following two features:
% % \begin{inparaenum}%[leftmargin=4mm]
% % \item \bf{Sentiments.} Opiner leverages sentiment analysis to offer insights to developers on whether a given
% % usage scenario is well-regarded or not in the forum posts. 
% % \item\bf{Statistics.} Opiner offers visualized representation of API usage in the summaries to 
% % facilitate quick insights into the API usage, which our study participants considered to be very useful for their learning and usage of the APIs. 
% % \end{inparaenum}
% % 
% % Ponzanelli et al.~\cite{Ponzanelli-PrompterRecommender-EMSE2014} developed an
% % Eclipse Plug-in that takes into account the source code in a given file as a
% % context and use that to search Stack Overflow posts to find relevant discussions
% % (i.e., \it{code to relevant information}). The relevant discussions are
% % presented in a multi-faceted ranking model. In two empirical studies, Prompter's
% % recommendations were found to be positive in 74\% cases. They also found that
% % such recommendations are `volatile' in nature, since the recommendations can
% % change at one year of distance.
% 
% 
% 
% 
% % \subsection{Software Code Search} 
% % Software development requires writing code to complete development tasks. Finding code examples similar to 
% % the task in hand can assist developers to complete the task quickly and efficiently. As such, a huge volume of research in software engineering 
% % has focused on the development and improvement of code search engines~\cite{Kim-Facoy-ICSE2018,Ponzanelli-PrompterRecommender-EMSE2014,
% % Gu-DeepCodeSearch-ICSE2018,McMillanGrechanik-Portfolio-ICSE2011,Chan-SearchingConnectedAPISubgraph-FSE2012,Haiduc-QueryReformulations-ICSE2013,
% % Lu-QueryExpansionViaWordnet-ICSME2015,Hill-NLBasedQueryRefinement-ICSME2014,Keivanloo-SpottingWorkingCodeExamples-ICSE2014,LvFei-CodeHow-ASE2015,Brandt-ExampleCentricProgramming-CHI2010}. 
% % The engines vary given the nature of input and output as well as 
% % the underlying searching, ranking, and visualization techniques. Based on input and output, the techniques can broadly be divided into following types: 
% % \begin{inparaenum}[(1)]
% % \item Code to code search, 
% % \item Code to relevant information search,
% % \item Natural language query to code search,
% % \item code snippet + natural language query to code search
% % \end{inparaenum}
% % 
% % Kim et al.~\cite{Kim-Facoy-ICSE2018} proposed FaCoy a \it{code-to-code search} engine, i.e., given as input a code snippet, 
% % the engine finds other code snippets that are \it{semantically} similar to the input code example. While our and FaCoY's 
% % goals remain the same, i.e., to help developers in their development tasks, we differ from each other with regards to both the 
% % outputs and the approaches. For example, given as input a code example in Stack Overflow post, we link it to an API name 
% % as mentioned in the textual contents of the post. In contrast, given as input a code example, FaCoY finds 
% % other similar code examples. 
% % % [1] Ponzanelli, L., G. Bavota, M. Di Penta, R. Oliveto, and M. Lanza. "Prompter: Turning the IDE into a self-confident programming assistant", Empirical Software Engineering, vol. 21, no. 5, 2016.
% % 
% % Natural language queries are used by leveraging text retrieval techniques to
% % find relevant code examples (i.e., \it{natural language query to code
% % search}).
% % McMillan et al.~\cite{McMillanGrechanik-Portfolio-ICSE2011} developed
% % Portfolio, a search engine to find relevant code functions by taking as input
% % a natural language search query that offers cues of the programming task in
% % hand. To assist in the usage of the returned functions, Portfolio also
% % visualizes their usages.
% % Hill et al.~\cite{Hill-NLBasedQueryRefinement-ICSME2014} proposes an Eclipse
% % plug-in CONQUER that takes as input a natural language query and finds
% % relevant source for maintenance by incorporating multiple feedback mechanisms
% % into the search results view, such as prevalence of the query words in the
% % result set, etc.
% % Lv et al.~\cite{LvFei-CodeHow-ASE2015} proposes CodeHow, a code search
% % technique to recognize potential APIs related to an input user query. CodeHow
% % first attempts to understand the input query, and then expands the query with
% % the potentially relevant APIs. CodeHow then performs code retrieval using the
% % expanded query by applying a Extended Boolean Model. The model considers the
% % impact of both text similarity and potential APIs during code search. In 26K
% % C\# projects from GitHub, CodeHow achieved a precision of 0.79 based on the
% % first returned relevant code snippet. In a controlled survey of Microsoft
% % developers, CodeHow was found to be effective.
% % Raghothaman et al.~\cite{Raghothaman-SWIMSyntehsizingWhatIMean-ICSE2016}
% % proposes SWIM that suggests code snippets by taking as input API-related
% % natural language queries.
% % The query does not need to contain framework specific keywords, because user
% % query is translated into APIs of interest using click-through data from Bing
% % search engine.
% % The tool was evaluated on C\#-related queries and was found to be effective,
% % responsive, and fast.
% % Keivanloo et al.~\cite{Keivanloo-SpottingWorkingCodeExamples-ICSE2014}
% % proposes a technique to spot working code examples among a set of code
% % examples. The approach combines clone detection with frequent itemset
% % mining~\cite{Agrawal-AssociationRuleLargeDB-ICVLD1994a} to detect popular
% % programming solutions.  The technique is specifically aimed to support
% % Internet-scale-code search engines, where usability is important. As such, the
% % technique focuses on three criteria: \begin{inparaenum}[(1)] \item the input
% % and output formats should be identical to the Internet-scale search engine,
% % \item the query should support free-form text, and \item the output should be
% % a ranked set of code examples.
% % \end{inparaenum} Brandt et al.~\cite{Brandt-ExampleCentricProgramming-CHI2010}
% % proposes to embed the results from web search engine into development
% % environment to create a task-specific search engine. They propose Blueprint, a
% % web search interface integrated into the Adobe Flex Builder developer
% % environment to help them find locate code.
% % Blueprint does this by automatically augmenting queries with code context and
% % by presenting a code-centric view of search results. A 3-month usage logs with
% % 2,024 users showed that the task-centric search interface significantly
% % changed how and when the users searched the Web.
% % 
% % 
% % The combination of code example/API structural knowledge and natural language queries are used to 
% % infer semantic meaning of the underlying programming task. Gu et al.~\cite{Gu-DeepCodeSearch-ICSE2018} proposes `Deep Code Search' by jointly embedding code snippets and natural language description into a high-dimensional 
% % vector space. Using the unified vector representation, code examples with purpose semantically similar to the natural language description can 
% % be found. The joint embedding allows semantic understanding of the purpose 
% % of the code and was found to be effective to retrieve relevant code snippets from large code base, such as GitHub. 
% % Chan et al.~\cite{Chan-SearchingConnectedAPISubgraph-FSE2012} proposes to recommend API code example by building API graph based on a simple text phrase, when the phrase may 
% % contain limited knowledge of the user. The API graph is buit by taking into account API invocations in client software. To optimize the traversing through the graph, they 
% % propose two refinement techniques. Comparison over Portfolio~\cite{McMillanGrechanik-Portfolio-ICSE2011} showed that the proposed API graph is superior.
% %  
% % While natural language queries are used extensively in many code search techniques, the queries may return sub-optimal results when they are not properly formulated.
% % Haiduc et al.~\cite{Haiduc-QueryReformulations-ICSE2013} proposes Refoqus, a machine learning engine that takes as input a search query and recommends 
% % a reformulation strategy for the input query to improve its performance. The engine is trained with a sample of queries and relevant results. The tool is evaluated 
% % against four baseline approaches used in natural language text retrieval in five open source software systems. The tool outperformed the baselines in 84\% of the cases.
% % Lu et al.~\cite{Lu-QueryExpansionViaWordnet-ICSME2015} proposes to use Wordnet~\cite{Miller-WordNet-CACM1995} to expand an input natural language search query against 
% % a code base. The use of Wordnet allows the expansion to also include semantically relevant keywords. Evaluation against the Javascript interpreter Rhino shows that the 
% % synonyms derived from Wordnet to expand the queries help recommend good alternative queries.
% % 
% % 
% % While finding relevant code example is important, an end-to-end engine can still be required to assist a developer to properly reuse the returned code example. 
% % Holmes et al.~\cite{Holmes-EndtoEndUserOfSourceCodeExamples-ICSME2009} outlines four case studies that involved end-to-end use of source code examples. 
% % The studies show that overhead and pitfalls involved in combining state-of-the-art techniques to support the use cases.
% % 
% % 
% % While the above work return code example as an output, we return an API name as mentioned in the forum post to associate to the code example found in the same post. 
% % Our end goals remain the same, i.e., to assist developers to complete in their coding tasks. However, while the above work focuses on the development of a code 
% % search engine, we focus on the generation of an API documentation. However, it is an interesting future avenue for us to explore the possibility of extending our API traceability 
% % technique by combining code search techniques. For example, we could employ methods similar to FaCoY to produce a semantic representation of a code example before attempting to link it to an API.
% % 
% % Zilberstein and Yahav~\cite{Zilberstein-Codota-ONWARD2016} proposed an approach 
% % to leverage code examples from forum posts to support auto code completion features in IDEs.
% % They built Codota, a tool that given a code context from the IDE, 
% % automatically searches forum posts to find most relevant code examples that can be relevant to the code context.
% % While the focus of both Opiner and Codota remains the same, i.e., assisting developers in their
% % development activities, Opiner differs from Codota as follows:
% % \begin{inparaenum}%[leftmargin=4mm]
% % \item \bf{Documentation Vs. Recommendation.} 
% % Opiner mines and documents API usage
% % scenarios. Codota provides recommendations to assist in code auto completion depending on the
% % code context in a developer IDE.
% % %\item \bf{Documentation Vs. IDE.} Opiner's focus is to offer improvements over developers' usage of formal and informal API documentation, 
% % %by producing automated summaries of usage scenarios from forum posts. Codota is a real-time assistant that aim to facilitate auto code-completion in the developers' IDE.
% % \item \bf{Diversity.} Opiner documentation can assist developers in their coding tasks, and support their diverse development 
% % scenarios, e.g., their selection of an API as well.
% % \end{inparaenum} Unlike Codota, Opiner supports the following two features:
% % \begin{inparaenum}%[leftmargin=4mm]
% % \item \bf{Sentiments.} Opiner leverages sentiment analysis to offer insights to developers on whether a given
% % usage scenario is well-regarded or not in the forum posts. 
% % \item\bf{Statistics.} Opiner offers visualized representation of API usage in the summaries to 
% % facilitate quick insights into the API usage, which our study participants considered to be very useful for their learning and usage of the APIs. 
% % \end{inparaenum}
% %\subsection{Code Summarization in Software Engineering}
% % The summarization of source code has been researched along
% % the following major dimensions:
% % \begin{inparaenum}
% % \item Summarization of code fragments,
% % \item Structural and textual descriptions of source code,
% % \item Summarization and recommendation of API documents, and 
% % \item Mining of usage patterns from execution traces.
% % \end{inparaenum}
% % 
% % \nd\bf{Summarization of Code Fragments.} When a code example can be too large to
% % get a quick insight, a number of recent research efforts can be used to summarize the code example, such as the selection and
% % presentation criteria of such code examples through developer
% % interviews~\cite{Ying-SelectionPresentationCodeExample-FSE2014} and eye tracking
% % experiment~\cite{Rodeghero-CodeSummarizationEyeTracking-ICSE2014}.
% % The focus of such summaries is to provide an
% % easy to understand representation of a code example in a search query result. 
% % Therefore, Ying and
% % Robillard~\cite{Ying-SelectionPresentationCodeExample-FSE2014} advocates the
% % needs to only show \it{interesting} parts of a code example in such summaries.
% % 
% % 
% % \nd\bf{Structural and Textual Summaries of Source Code.} Poorly documented source code can make APIs hard to
% % learn~\cite{Robillard-APIsHardtoLearn-IEEESoftware2009a,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a}.
% % To address this problem research in software engineering has 
% % \begin{inparaenum}[(1)]
% % \item produced structural summary of code
% % base~\cite{Murphy:summarization,murphy:context}. 
% % \item recommended the right code snippets for a
% % development task in hand~\cite{Holmes-Strathcona-TSE2006a}.
% % \item produced natural language summaries of source
% % code by leveraging call graphs~\cite{Moreno13}, method
% % contexts~\cite{McBurney14}, identifier and variable names in
% % methods~\cite{Sridhara-MethodSummary-ASE2010}, and by combining both structural
% % and lexical information in source code~\cite{Haiduc:Summarization}.
% % \end{inparaenum}
% % % 
% % % Natural language summaries have been investigated for software
% % % documentation~\cite{Rastkar:2014,murphy:context,Holmes-Strathcona-TSE2006a, anvik:context} and
% % % source code~\cite{Sridhara-MethodSummary-ASE2010,Moreno13,McBurney14,Guerrouj15-nier}.
% % % Murphy \cite{Murphy:summarization} proposed two techniques to produce
% % % structural summary of source code. Storey et al.~\cite{Storey:tagging}
% % % analyzed the impact of tags and annotations in source code. The
% % % summarization of source code element names (types, methods) has been
% % % investigated by leveraging both structural and
% % % lexical information of the source code~\cite{Haiduc:Summarization}, by focusing on
% % % contents and call graphs of Java classes~\cite{Moreno13}, based on the
% % % identifier and variable names in methods~\cite{Sridhara-MethodSummary-ASE2010}.
% % % More recently McBurney and McMillan proposed a technique to generate automatic
% % % documentation via the source code summarization of method context~\cite{McBurney14}. The notion of context is very important for developers because it helps understand why code elements exist and the rationale behind their
% % % usage in the software \cite{Ekwa-StudyUnfamiliarAPIs-ICSE2012,Sillito-AskingandAnsweringQuestions-TSE2008a,SimCH98}.  
% % The usage summaries in Opiner differ from the above work as
% % follows. 
% % \begin{description}
% %   \item \bf{Summarization Definition.} The above work consider a summary of a
% %   code example as a natural language or structural description of what the code
% %   does. We consider a summary as a set of usage scenarios of an API that are relevant.
% %   \item \bf{Summary Description.} The above work produce a textual description of a code example by 
% %   taking into account the variable and method names in the code example. 
% %   We produce a textual description of a code
% %   example by collecting textual contents from a forum post where the code example is found.
% %   \item \bf{Summarization Contents.} The above work produce summaries by using 
% %   structural or lexical contents or a combination of both types of contents. In our four
% %   summaries, we combine
% %   structural information from the code example with lexical contents from forum post.
% % \end{description}
% % % In
% % % our previous work, we proposed summarization techniques for API reviews and
% % % found that they were useful to support developers in their selection of
% % % APIs~\cite{Uddin-OpinerReviewAlgo-ASE2017,Uddin-OpinerReviewToolDemo-ASE2017}.
% % % Our findings in this paper confirmed that developers also require different
% % % types of API usage scenario summaries.
% % 
% % \nd\bf{Summarizing and Recommending API Documents.} Our goal to produce API usage summaries is to assist in the documentation
% % efforts of an API, such that developers can leverage those to complete their
% % development tasks. This same goal can also be achieved when a developer can be
% % shown the right forum posts that are related to his development tasks, such as
% % \begin{inparaenum}[(1)]
% % \item by automatically finding relevant questions in Stack Overflow given a
% % query~\cite{BowenXu-CrossLanguageRelevantQuestion-EMSE2017,BowenXu-PredictSemanticLinkableKnowledgeInForumsCNN-ASE2016},
% % and
% % \item by summarizing the most \it{relevant} information from a
% % different forum posts or from API documentation itself as an answer to a query
% % (that describes the development task in natural language
% % queries)~\cite{BowenXu-AnswerBot-ASE2017,YuanTian-APIBot-ASE2017}.
% % \end{inparaenum}
% % 
% % Our user studies show that the summaries in Opiner can be one way to address the
% % problems developers face while using forum posts for API-related tasks,
% % i.e., lack of discoverability and quick insights). In our concept-based
% % summaries, we cluster conceptually similar usage scenarios in a `See Alsos'
% % section. Unlike AnsweBot~\cite{BowenXu-AnswerBot-ASE2017} or
% % APIBot~\cite{YuanTian-APIBot-ASE2017} above, Opiner does not support
% % the discoverability of usage scenarios via a search query. Adding such utility
% % features in Opiner can assist the users in Opiner to find the relevant usage
% % summaries with relative ease.
% % 
% % %\subsection{Mining API Usage Patterns}
% % \nd\bf{Mining Usage Patterns from Execution Traces.} Dynamic analysis is used on the execution traces to detect usage
% % patterns~\cite{Lo-MiningHierarchicalScenarioBasedSpec-ASE2009,Lo-MiningIterativePatterns-SIGKDD2007,Fahland-MiningBranchingTimeScenarios-ASE2013,Safyallah-PatternMiningDynamicAnalysis-ICPC2006}.
% % The techniques instrument software and collect execution traces by running the
% % software for relevant task scenarios. Static analysis is used on the version control
% % data of software to find API usage
% % concepts~\cite{Uddin-TemporalApiUsage-ASE2011,Uddin-TemporalApiUsage-ICSE2012,Robillard-AutomaticSuggestionProgramNavigation-FSE2005,Robillard-RecommendChangeClusters-JournalSoftwareMaintain2010a,Robillard-RepresentingConcern-PhDThesis2003}.
% % To the best of our knowledge, ours is the first technique to mine API usage
% % scenarios from developer forums by combining code examples to developer
% % reactions. We parse code examples using static analyses. Therefore, we do not
% % require instrumented application software to find usage scenarios for APIs.
% % Unlike patterns derived from the execution traces of a software, we 
% % investigate patterns of similar code examples in the mined scenarios. 
% % 
% % % We have previously developed a technique to automatically mine temporal
% % % API usage concepts from version histories of client software of an
% % % API~\cite{Uddin-TemporalApiUsage-ICSE2012}. Our concept-based summaries differ from~\cite{Uddin-TemporalApiUsage-ICSE2012}
% % % because the summaries are produced based on the code examples mined from Stack Overflow. As such the algorithms to detect concepts differ between the two works. For example, in~\cite{Uddin-TemporalApiUsage-ICSE2012}, 
% % % we incorporate time-based ordering of Principal Component Analysis (PCA) to detect concepts. In our concept-based summaries, we leverage static code analysis techniques with frequent itemset 
% % % mining to detect concepts.   
% % 
% % % In addition, unlike the temporal API usage concepts in~\cite{Uddin-TemporalApiUsage-ICSE2012} 
% % % that show  
% % %  as follows: \begin{inparaenum}
% % % \item We produced the temporal API usage concepts by automatically mining the
% % % version histories of client software where the API was used. Our concept-based
% % % summaries are produced based on the code examples mined from Stack Overflow.
% % % \item We produced patterns of API usage concepts in our temporal API usage
% % % mining, by showing how a set of concepts can be used in sequence. In our
% % % concept-based summaries, we cluster conceptually similar code examples that may
% % % not follow a predefined order of execution.
% % % \end{inparaenum}
% % % Our type-based summaries adhere to the Javadoc format, but
% % % differentiate from both Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}
% % % and API Insight~\cite{Treude-APIInsight-ICSE2016} by including sentiments as reactions in the usage summaries 
% % % as well as by producing natural language description of the code example. 
% % % 
% % %  as follows:
% % % \begin{description}
% % % \item [Live API documentation
% % % (Baker)~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}:]
% % % The Baker tool provides a browser extension that can annotate the pages of an
% % % API type in a Javadoc with the link of a forums post where a code example for
% % % the API type was found. In Opiner, we put all the API types in one single page.
% % % All the usage scenarios of a given API type are provided under a collapsible
% % % box under the type. The API type itself functions as toggle button, i.e., by
% % % clicking on it a user can either see all the code examples or collapse the view
% % % to hid the scenarios. In this way, we ensured that the user can see all the
% % % usage scenarios of the API types in one single page, thereby adhering to the
% % % venerable single page documentation style of Python documentation. Moreover, while
% % % Baker simply provides a link to a forum post where the code example is found,
% % % our tool Opiner shows a usage scenario. A usage scenario not only contains a
% % % code example, but also shows other relevant information, such as, short summary
% % % description and positive and negative opinions of other developers towards the
% % % code example. Such information thus can provide instant insight about the
% % % usefulness of a code example. For example, a code example with mostly negative
% % % opinions is unlikely to be useful and thus can be avoided.  
% % % 
% % % \item[API insight~\cite{Treude-APIInsight-ICSE2016}:] Treude and
% % % Robillard~\cite{Treude-APIInsight-ICSE2016} proposed a tool to annotate the
% % % Javadocs of API types with key insights about them mined from Stack Overflow.
% % % Such insights are collected from the textual contents of the forum posts where
% % % the API types are discussed. It is not necessary for a code example of an
% % % API type to be present in the same forum post from where the insight is mined.
% % % In contrast, for a usage scenario of an API type in Opiner, all of the following
% % % five items are considered as required: \begin{inparaenum}
% % % \item a code example,
% % % \item a summary description, 
% % % \item a title, and 
% % % \item positive and negative opinions.
% % % \end{inparaenum} The positive and negative opinions in
% % % Opiner are collected from comments to a forum post (where a code example was
% % % found). Opiner's focus is suited to assist developers in their programming tasks
% % % by showing readily available code snippets of an API as well as in their instant
% % % decision process on whether a code snippet is a good fit. 
% % % \end{description}
% % 
% % 
% % % In our previous study~\cite{Uddin-TemporalApiUsage-ICSE2012}, we mined API usage
% % % concepts from the version histories of client software that used an API of our
% % % interest. We observed that developers in multiple unrelated software often used
% % % a pre-defined set of of the same API types to complete a development task. 
% % % We also observed patterns of concept usage. For
% % % example, to send or receive messages over HTTP using the HttpClient API, 
% % % a developer would first need to establish an HTTP connection 
% % % followed by the usage of the HttpGet or HttpPost method to send or receive message.
% % % 
% % % \subsection{Sentiment Analysis in Software Artifacts} Ortu et
% % % al.~\cite{Ortu-AreBulliesMoreProductive-MSR205} observed that bullies are not more productive than others in a software development team.
% % % M\"{a}ntyl\"{a}  et al.~\cite{Mika-MiningValenceBurnout-MSR2016} correlated VAD
% % % (Valence, Arousal, Dominance) scores~\cite{Warriner-VadLexicons-BRM2013} in
% % % Jira issues with the loss of productivity and burn-out in software engineering
% % % teams. Pletea et al.~\cite{Pletea-SecurityEmotionSE-MSR2014} observed that
% % % security-related discussions in GitHub contained more negative comments. Guzman et
% % % al.~\cite{Guzman-SentimentAnalysisGithub-MSR2014} found that GitHub
% % % projects written in Java as well as the comments posted on Mondays have more
% % % negative comments, while the developers in a distributed team are more positive.
% % % Guzman and Bruegge~\cite{Guzman-EmotionalAwareness-FSE2013} summarized emotions
% % % expressed across collaboration artifacts in a software team (bug reports, etc.) using LDA~\cite{Blei-LDA-JournalMachineLearning2003} and sentiment analysis.
% % % Murgia et al.~\cite{Murgia-DoDevelopersFeelEmotion-MSR2014}
% % % labelled comments from Jira issues using Parrot's framework~\cite{Parrot-EmotionsSocialPsychology-PsychologyPress2001}.
% % % %They observed only 46.11$\pm$5\% agreement of the comments where
% % % %the raters agreed on the same rating, and even lesser agreement when more
% % % %contexts were added to the comment.
% % % Jongeling et al.~\cite{Jongeling-SentimentAnalysisToolsSe-ICSME2015} compared four sentiment
% % % tools on comments posted in Jira while
% % % %: SentiStrength~\cite{Thelwall-Sentistrength-ASICT2010},
% % % %Alchemy~\cite{website:alchemy}, Stanford NLP~\cite{Socher-Sentiment-EMNLP2013},
% % % %and NLTK~\cite{website:nltk}. While NLTK and SentiStrength showed better
% % % %accuracy, there were little agreements between the two tools.
% % % Novielli et al.~\cite{Novielli-ChallengesSentimentDetectionProgrammerEcosystem-SSE2015}
% % % analyzed the sentiment scores from the StentiStrength in Stack Overflow posts.
% % % They observed that developers express emotions towards the technology, not towards other developers.
% % % They found that the tool was unable to detect domain-dependent sentiment words (e.g., bug). 
% % % The development of Opiner was motivated by the findings of the impact of
% % % sentiments in software teams and repositories. While the major focus of Opiner
% % % usage summaries was to summarize the code usage examples, each usage such
% % % example was accompanied by positive and negative opinions.
% % %\Foutse{how do all these work connect to your work...you need to explain a
% % % bit...}
% % % These findings indicate that the mere application of an off-the-shelf tool may
% % % be insufficient to capture the complex sentiment found in the software
% % % artifacts.
% % 
% % 
% % % \subsection{APIs in Informal Documentation}
% % % Parnin et al.~\cite{Parnin2012} have examined API classes discussed in
% % % Stack Overflow using heuristics based on exact matching of class names with words in posts (title, body, snippets, etc.).
% % % Similarly, Kavaler et al.~\cite{Kavaler-APIsUsedinAndroidMarket-SOCINFO2013} have analyzed the relationship between API usage and their related Stack Overflow discussions. Both studies found a positive relationship between the volume of Stack Overflow discussions and API usages.
% % % Recently, Linares-Vasquez et al.~\cite{Linares-Vasquez-2014,Guerrouj15-saner} investigated the relationship between API changes and developer discussions. Dagenais et al. proposed techniques to trace API code terms in documentation~\cite{Dagenais-RecoDocPaper-ICSE2012a}. This paper contributes to this line of work as we also propose techniques to associate code examples to APIs terms. Other relevant studies on the same topic include~\cite{Rigby-CodeElementInformalDocument-ICSE2013,Subramanian-LiveAPIDocumentation-ICSE2014,BettenburgCSMR2012},
% % % and in emails~\cite{Bacchelli-LinkEmailSourceCode-ICSE2010a}.
% % 
% % 
% % %\nd\bf{Defect and Feature Traceability.}
% % %Hayes et
% % %al.~\cite{Hayes-TraceabilityAdvancingStudy-IEEETSE2006} used three IR
% % %algorithms (LSI, VSM, and VSM with thesaurus) to establish links between
% % %a high and low-level
% % %requirement descriptions.
% % %Lormans et al.~\cite{Lormans-TraceabilityLSIReconstructing-CSMR2006} used LSI to find
% % %relationships between requirements, tests, and design documents.
% % %Baysal et
% % %al.~\cite{Baysal-CorrelateSocialInterationsReleaseHistory-MSR2007} correlated
% % %emails in mailing lists and software releases by linking emails with the source
% % %code. Types and variable names in the source code were matched against natural
% % %language queries to assist in feature
% % %location~\cite{PoshyvanykMarcus-LSIwithFCA-ICPC2007a,Eisenbarth-FeatureLocation-TSE2003,Marcus-TraceabilityLSI-ICSE2003}.
% % %Given as input a bug report, Hipikat~\cite{CubranicGail-Hipikat-TSE2006} finds relevant source code and other artifacts (e.g., another bug report).
% % %Subsequent techniques linked a bug fix
% % %report to its related code
% % %changes~\cite{Wu-RelinkBugChange-FSE2011,Nguyen-LinkBugReportFixes-FSE2012a},
% % %or detected duplicate bug reports~\cite{Nguyen-DuplicateBugReport-ASE2012}.
% % 
% % % \subsection{Code Term Traceability Recovery}
% % % Recodoc~\cite{Dagenais-RecoDocPaper-ICSE2012a} resolves code terms in the formal
% % % documentation of a project to its exact corresponding
% % % element in the code of the project.
% % % Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}
% % % links code terms in the code snippets
% % % of Stack Overflow posts to an API/framework whose name was used to tag the
% % % corresponding thread of the post.
% % % ACE~\cite{Rigby-CodeElementInformalDocument-ICSE2013} resolves Java code terms
% % % in forum textual contents of posts using island
% % % grammars~\cite{Moonen-IslandParser-WCRE2001}. Bacchelli et
% % % al.~\cite{Bacchelli-LinkEmailSourceCode-ICSE2010a} developed Miler to determine
% % % whether a development email of a project contains the
% % % mention of a given source code element. They compared information retrieval (IR)
% % % techniques (LSI~\cite{Marcus-TraceabilityLSI-ICSE2003}
% % % and VSM~\cite{Manning-IRIntroBook-Cambridge2009}) against lightweight techniques
% % % based on regular expressions. 
% % % %They found that the lightweight techniques outperformed the IR techniques.
% % % Prior to Miler, LSI was also used by Marcus et al.~\cite{Marcus-TraceabilityLSI-ICSE2003},
% % % and VSM was compared with a probabilistic IR model by Antoniol et
% % % al.~\cite{Antoniol-TraceabilityCodeDocumentation-IEEETSE2002}.
% % % % None of
% % % % them~\cite{Bacchelli-LinkEmailSourceCode-ICSE2010a,Marcus-TraceabilityLSI-ICSE2003,Antoniol-TraceabilityCodeDocumentation-IEEETSE2002},
% % % % addressed the ambiguity that a mentioned code term may
% % % % match more than one code element.
% % % Tools and techniques have been proposed to leverage code traceability
% % % techniques, e.g., linking software artifacts where a code
% % % term is found~\cite{Inozemtseva-IntegrateSEArtifacts-ICSE2014},
% % % associating development
% % % emails with the source code in developers' IDE~\cite{Bacchelli-Remail-ICSM2011},
% % % recommending posts in
% % % Stack Overflow relevant to a given code context in the
% % % IDE~\cite{Ponzanelli-PrompterRecommender-MSR2014}. Opiner extends to this line
% % % of work by proposing a heuristic-based technique to associate a code example in
% % % forum posts to one or more APIs. 
% % 
% % % \subsection{Summarization in Software Engineering}
% % % 
% % % Natural language summaries have been investigated for software
% % % documentation~\cite{Rastkar:2014,murphy:context,Holmes-Strathcona-TSE2006a, anvik:context} and
% % % source code~\cite{Sridhara-MethodSummary-ASE2010,Moreno13,McBurney14,Guerrouj15-nier}.
% % % Murphy \cite{Murphy:summarization} proposed two techniques to produce
% % % structural summary of source code. Storey et al.~\cite{Storey:tagging}
% % % analyzed the impact of tags and annotations in source code. The
% % % summarization of source code element names (types, methods) has been
% % % investigated by leveraging both structural and
% % % lexical information of the source code~\cite{Haiduc:Summarization}, by focusing on
% % % contents and call graphs of Java classes~\cite{Moreno13}, based on the
% % % identifier and variable names in methods~\cite{Sridhara-MethodSummary-ASE2010}.
% % % More recently McBurney and McMillan proposed a technique to generate automatic
% % % documentation via the source code summarization of method context~\cite{McBurney14}. The notion of context is very important for developers because it helps understand why code elements exist and the rationale behind their
% % % usage in the software \cite{Ekwa-StudyUnfamiliarAPIs-ICSE2012,Sillito-AskingandAnsweringQuestions-TSE2008a,SimCH98}.  The selection and presentation of source code summaries have been explored through
% % % developer interviews~\cite{Ying-SelectionPresentationCodeExample-FSE2014}, as well as eye
% % % tracking experiment~\cite{Rodeghero-CodeSummarizationEyeTracking-ICSE2014}. In
% % % our previous work, we proposed summarization techniques for API reviews and
% % % found that they were useful to support developers in their selection of
% % % APIs~\cite{Uddin-OpinerReviewAlgo-ASE2017,Uddin-OpinerReviewToolDemo-ASE2017}.
% % % Our findings in this paper confirmed that developers also require different
% % % types of API usage scenario summaries.
% % 
% % 
% % % \subsection{Code Completion Using Crowd-Sourced API Code
% % % Examples} Zilberstein and Yahav~\cite{Zilberstein-Codota-ONWARD2016} proposed an approach 
% % % to leverage code examples from forum posts to support auto code completion features in IDEs.
% % % They built Codota, a tool that given a code context from the IDE, 
% % % automatically searches forum posts to find most relevant code examples that can be relevant to the code context.
% % % While the focus of both Opiner and Codota remains the same, i.e., assisting developers in their
% % % development activities, Opiner differs from Codota as follows:
% % % \begin{inparaenum}%[leftmargin=4mm]
% % % \item \bf{Summary Vs. Recommendation.} 
% % % Opiner mines and summarizes API usage
% % % scenarios to assist in API documentation. Codota provides recommendations to assist in code auto completion depending on the
% % % code context in a developer IDE.
% % % %\item \bf{Documentation Vs. IDE.} Opiner's focus is to offer improvements over developers' usage of formal and informal API documentation, 
% % % %by producing automated summaries of usage scenarios from forum posts. Codota is a real-time assistant that aim to facilitate auto code-completion in the developers' IDE.
% % % \item \bf{Diversity.} Opiner summaries can assist developers in their coding tasks, and support their diverse development 
% % % scenarios, e.g., their selection of an API as well.
% % % \end{inparaenum} 
% % % 
% % % Unlike Codota, Opiner supports the following two features:
% % % \begin{inparaenum}%[leftmargin=4mm]
% % % \item \bf{Sentiments.} Opiner leverages sentiment analysis to offer insights to developers on whether a given
% % % usage scenario is well-regarded or not in the forum posts. 
% % % \item\bf{Statistics.} Opiner offers visualized representation of API usage in the summaries to 
% % % facilitate quick insights into the API usage, which our study participants considered to be very useful for their learning and usage of the APIs. 
% \end{inparaenum}

==> DocBotSANER2021 (Camera Ready)/study-results.tex <==
\section{Automatic Detection of The Smells}\label{sec:model}
The responses from the survey validate our catalog of API documentation smells. 
The perceived negative impact of the smells on developers' productivity, as evidenced by the responses from our survey participants, necessitates the 
needs to fix API documentation by removing the smells. To do that, we first need to detect the smells automatically in the API documentation. The automatic detection offers 
two benefits: (1) we can use the techniques to automatically monitor and warn about bad documentation quality and (2) we can design techniques 
to fix the smells based on the detection. In addition, manual effort can also be made for improving detected examples. 
With a view to determine the feasibility of techniques to detect API documentation smells using our benchmark, 
we answer three research questions:
\begin{enumerate}[label=RQ\arabic{*}., start = 3, leftmargin=25pt]
  \item How accurate are rule-based classifiers to automatically detect the documentation smells?
  \item Can the shallow machine learning models outperform the rule-based classifiers?
  \item Can the deep machine learning models outperform the other models?
  %\anindya{The third RQ assumes that shallow learning techniques will outperform rule-based ones. We may rather say "outperform the other techniques".}
  %\item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}
%\subsection{Performance Metrics}
The shallow and deep learning models are supervised, for which we used 5-fold
iterative stratified cross-validation as
recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}.
Traditional $k$-fold cross-validation is a statistical method of evaluating
machine learning algorithms which divides data into $k$ equally sized folds and
runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each
iteration, each of the $k$ folds is used as the held-out set for validation
while the remaining $k-1$ folds are used as training sets. Stratified
cross-validation is used to make sure that each fold is an appropriate
representative of the original data by producing folds where the proportion of
different classes is maintained \cite{stratified_cross_validation_paper}.
However, stratification is not sufficient for multi-label classification
problems as the number of distinct labelsets (i.e., different combinations of
labels) is often quite large. For example, there can be 32 combinations of
labels in our study as there are 5 types of documentation smells. In such cases,
original stratified $k$-fold cross-validation is impractical since most groups
might consist of just a single example. Iterative stratification, proposed by
\cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy
approach of selecting the rarest groups first and adding them to the smallest
folds while splitting. 

We report the performances using four standard metrics in information
retrieval~\cite{Manning-IRIntroBook-Cambridge2009}. Accuracy ($A$) is the ratio of
correctly predicted instances out of all the instances. Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given smell.
Recall ($R$) represents the ratio of the number of correctly predicted instances
and all instances belonging to a given class. F1-score ($F1$) is the harmonic mean of
precision and recall.

{\scriptsize
\begin{eqnarray*}
P  = \frac{TP}{TP+FP},~
R = \frac{TP}{TP+FN},~
F1 = 2*\frac{P*R}{P+R},~
A = \frac{TP+TN}{TP+FP+TN+FN}
\end{eqnarray*}}
TP = Correctly classified as a smell, 
FP = Incorrectly classified as a smell, TN = Correctly classified as not a smell, 
FN = Incorrectly classified as not a smell. 

% We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

% \begin{inparaenum}[(a)]
% % \item\bf{Iterative Stratified Cross-Validation}

% % \item\bf{Exact Match Ratio}
% % In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

% % \begin{equation}
% % EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
% % \label{eq:EMR}
% % \end{equation} %&

% % {$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
% % }


% % \item\bf{Hamming Loss}
% % Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
% % \begin{equation}
% % HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
% % \end{equation}

% % {$N$ is the total number of data, $L$ is the total number of labels.}

% \item\bf{Accuracy}
% Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
% \begin{equation}
% A = \frac{TP+TN}{TP+FN+TN+FP}
% \label{eq:acc}
% \end{equation}

% {$TP$ is the number of true positives, $FN$ is the number of false
% negatives, $FP$ is the number of false positives, $TN$ is the number of true
% negatives.}


% \item\bf{Precision}
% Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
% \begin{equation}
% P  = \frac{TP}{TP+FP} 
% \label{eq:precision}
% \end{equation} %&


% \item\bf{Recall}
% Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

% \begin{equation}
%  R = \frac{TP}{TP+FN}
%  \label{eq:recall}
%  \end{equation} 
 

% \item\bf{F1-score}
% F1-score is the harmonic mean of precision and recall.
% \begin{equation}
% F1 = \frac{2\cdot P\cdot R}{P+R}
% \label{eq:f-score}    
% \end{equation}

% \end{inparaenum}

\subsection{Performance of Rule-Based Classifiers (RQ3)}\label{sec:rule-based}
Based on manual analysis of a statistically significant random sample of our benchmark dataset (95\% confidence interval and 5 levels), 
we designed six metrics to establish five rule-based classifiers as described below. 
\subsubsection{Rule-based Metrics}
\label{subsubsec:rule-based-metrics}
%\subsubsection{Approach}
%\gias{discuss the studied features, put the feature summaries in a table}
%discuss the features, group the features into a set of feature dimensions.
\begin{inparaenum}[(a)]
\item\it{Documentation Length.} We use the length of every documentation in order to capture the extensiveness of the bloated documentations.
\item\it{Readability Metrics.} We measure Flesch readability metrics \cite{flesch_readability_paper} for the documentations 
to analyze the understandability of documentation. This feature might be useful to detect tangled documentations.
\item\it{Number of Acronyms and Jargons.} Since acronyms and jargons increase the
complexity of a reading passage \cite{jargon_paper_1}, we use the number of
acronyms and jargons in every documentation to detect the tangled documentation.
%by estimating the understandability.
\item\it{Number of URLs} is computed because URLs are hints of possible fragmentation in the
documentation.
\item\it{Number of function, class, and package name mentioned} in documentation is computed to capture
excess structural information smell.
\item\it{Edit Distance.} The edit distance (i.e., measure of dissimilarity) between the
description of a lazy documentation and its' corresponding unit definition
(i.e., method prototype) can be smaller than non-lazy
documentations. We calculate the Levenshtein distance
\cite{edit_distance_levenshtein_paper} between the documentation description and
method prototype.
%\item\bf{Average Cosine Similarity.} We calculate the avg. cosine similarity of the documentations’ description. For this, we calculate the cosine similarities between each possible pair of that documentation and take their avg value for normalization. This feature will help to detect redundancy in the documentations.
\end{inparaenum}

\subsubsection{Rule-based Classifiers}
\fig\ref{fig:rule_based_classification_flowchart} shows flowchart of the rule-based classification approach.
For each metric, we study average, $25^{th}$, $50^{th}$, $75^{th}$, and $90^{th}$ percentiles as thresholds. 
    



%%%%%%%%%%%%%%%%
%% Rule based model flowchart
%%%%%%%%%%%%%%%
\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  \hspace*{-.3cm}%
   \includegraphics[scale=.55]{new_images/Rulebased_Flowchart.png}
 % \vspace{-4mm}
  \caption{Flowchart of rule-based classification approach.}

  \label{fig:rule_based_classification_flowchart}
\vspace{-4mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsubsection{Results}
\label{subsec:results_of_rulebased_baselines}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Table of rule-based  Baseline models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\caption{Class-wise performance of rule-based baseline models by the metric thresholds (P stands for percentile)}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{p{.6cm}|lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\
\midrule
{\textbf{Model}}   & \bf{Threshold}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\
\midrule
\multirow{5}{=}{\textbf{Rule Based}}
& {\textbf{AVG}}
& {.77} & {.38} & {.86} &{.52} %bloated
& {.58} & {.39} & {.71} &{.51} %lazy
& {.68} & {.35} & {.34} &{.34} %excess
& {.49} & {.13} & {.18} &{.15} %tangled
& {.65} & {.33} & {.52} & {.40} %fragmented
\\ %\hline
& {\textbf{25P}}
& {.39} & {.18} & {.64} &{.29} %bloated
& {.96} & {.96} & {.93} & \bf{.95} %lazy
& {.67} & {.38} & {.30} &{.34} %excess
& {.54} & {.09} & {.09} &{.09} %tangled
& {.52} & {.31} & {.90} &\bf{.47} %fragmented
\\ %\hline
& {\textbf{50P}}
& {.64} & {.28} & {.79} &{.41} %bloated
& {.77} & {.55} & {.84} &{.66} %lazy
& {.75} & {.37} & {.50} & \bf{.42} %excess
& {.45} & {.20} & {.40} &{.26} %tangled
& {.61} & {.34} & {.71} &{.46} %fragmented
\\ %\hline
& {\textbf{75P}}
& {.89} & {.56} & {.93} &{.70} %bloated
& {.52} & {.36} & {.67} &{.47} %lazy
& {.65} & {.32} & {.31} &{.31} %excess
& {.37} & {.25} & {.75} &{.37} %tangled
& {.67} & {.29} & {.27} &{.28} %fragmented
\\ %\hline
& {\textbf{90P}}
& {.95} & {.97} & {.85} & \bf{.90} %bloated
& {.37} & {.30} & {.56} &{.39} %lazy
& {.75} & {.50} & {.17} &{.25} %excess
& {.33} & {.26} & {.96} & \bf{.41} %tangled
& {.72} & {.27} & {.10} &{.15} %fragmented
\\ %\hline
\bottomrule
%{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
%{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\
%\hline
\end{tabular}
%}
\label{table_individual_performance_baseline}
%\end{center}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Table \ref{table_individual_performance_baseline}, we reported the
performances of the baseline models for each documentation smell. Different
thresholds of features achieved higher performance for different documentation
smells. For example, taking 90\textsuperscript{th} percentiles of the features’
values, baseline model achieved the higher performance for bloated documentation
detection, while lazy and excess structural information smell detection required
25\textsuperscript{th} percentile and 50\textsuperscript{th} percentile,
respectively. Notably, the performance of the baseline models in detecting
bloated (.90 F1-score) and lazy (F1 = .95) documentation were higher than
detecting excess structural info (F1 = .42), tangled (F1 = .41), and
fragmented (F1 = .47) documentations. 
%Clearly, bloated and lazy documentation
%were captured  better by the rule-based features (e.g., documentation
%length and edit distance) than the other documentation smells.


\subsection{Performance of Shallow Learning Models (RQ4)}\label{sec:shallow-learning}
\subsubsection{Shallow Learning Models}
%We applied both traditional and deep learning algorithms to detect documentation smells. 
Since documentation smell detection is multi-label classification problem, we
employed different decomposition approaches: One-Vs-Rest (OVR), Label Powerset
(LPS), and Classifier Chains
(CC)~\cite{multilabel_decomp_1_MultilabelClassificationAnOverview,multilabel_decomp_2_AReviewOnMultilabelLearning,multilabel_decomp_3_ATutorialOnMultilabelClassification,multilabel_decomp_4_LearningFromMultilabelData}
with Support Vector Machine (SVM) \cite{SVM_SupportVectorNetworks} as the base
estimator. We chose SVM and OVR-SVM since those are successfully used for
multi-label text classification \cite{SVM_multi_1_AKernelMethodForMultilabelled,
SVM_multi_2_TextCategorizationWithSVM,svm_text_classification_1,
svm_text_classification_2,multilabel_decomp_1_MultilabelClassificationAnOverview}.
Each model trains a single classifier per class, with the samples of that class
as positive samples and all other samples as negatives. Each
individual classifier then separately gives predictions for unseen data.
We used linear kernel for the SVM classifiers as recommended by earlier works
\cite{svm_linear_kernel_paper_1, svm_linear_kernel_paper_2}.
\cite{svm_rbf_1_AComparisonStudyOfDifferentKernelFunctions,
svm_rbf_2_APracticalGuideToSVM}.   We also evaluated adapted approaches like
Multi label (ML) $k$NN \cite{MLkNN_ALazyLearningApproach} in this study. It
finds the $k$ nearest neighborhood of an input instance using $k$NN, then uses
Bayesian inference to determine the label set of the instance. We studied this
method because it has been reported to achieve considerable performance for
different multi-label classification tasks in previous studies
\cite{MLkNN_ALazyLearningApproach,
mlknn_MultilabelTextClassificationUsingSemanticFeatures}. For each algorithm, we
picked the best model using standard practices, e.g., hyper parameter tuning in
SVM as recommended by Hsu~\cite{Hsu-PracticalSVM-Misc2010}, choice of K in
ML-kNN as recommended by
\cite{mlknn_MultilabelTextClassificationUsingSemanticFeatures}.
% 
% %%%, and deep learning models like Bi-LSTM \cite{bi_lstm_BidirectionalRecurrentNeuralNetworks}, and BERT \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. 
% 
% %\subsubsection{OVR-SVM}
% %\label{subsubsec:ovr_svm}
% \begin{inparaenum}[(a)]
% \item\bf{One-Vs-Rest (OVR)} is a heuristic method that works by decomposing the
% multi-label classification problem into multiple independent binary
% classification problems (one per class)
% \cite{multilabel_decomp_1_MultilabelClassificationAnOverview,
% multilabel_decomp_3_ATutorialOnMultilabelClassification}. It trains a single
% classifier per class, with the samples of that class as positive samples and all
% other samples as negatives. All the independent classifiers then separately give
% individual class predictions for unseen data. We evaluated One-Vs-Rest (OVR)
% approach with SVM (as the base estimator) for detecting documentation smells.
% One-Vs-Rest support vector machine (OVR-SVM) has been successfully applied in
% several problems \cite{SVM_multi_1_AKernelMethodForMultilabelled,
% SVM_multi_2_TextCategorizationWithSVM,
% multilabel_decomp_1_MultilabelClassificationAnOverview}. We used linear kernel
% for the SVM classifiers as recommended by earlier works
% \cite{svm_linear_kernel_paper_1, svm_linear_kernel_paper_2}.
% \cite{svm_rbf_1_AComparisonStudyOfDifferentKernelFunctions,
% svm_rbf_2_APracticalGuideToSVM}.
% 
% % \subsubsection{LPS-SVM} \label{subsubsec:lps_svm}
% \item\bf{Label Power Set (LPS)} treats every combination of labels as a new
% class and approaches in a multiclass classification manner
% \cite{LearningMultiLabelSceneClassification}. As a result, this method has high
% computational complexity. However, it is capable of taking label correlation
% into account. We used SVM (with linear kernel) as the base estimator of the
% Label Power Set method \cite{SVM_multi_1_AKernelMethodForMultilabelled,
% SVM_multi_2_TextCategorizationWithSVM,svm_linear_kernel_paper_1}.
% 
% 
% % \subsubsection{CC-SVM} \label{subsubsec:cc_svm}
% \item\bf{Classifier Chains (CC)} constructs a chain of binary classifiers, where
% every classifier uses the predictions of all the previous classifiers of the
% chain \cite{CC_1_ClassifierChainsForMultilabel,
% CC_2_ClassifierChainsForMultilabel}. This way the method can take label
% correlations into account. We constructed a Classifier Chain (CC) of SVMs and
% evaluated its’ performance for documentation smell detection.
% 
% 
% 
% % \subsubsection{ML-$k$NN} \label{subsubsec:ml_knn}
% \item\bf{Multi-label $k$ Nearest Neighbors (ML-$k$NN)} is derived from the
% traditional $k$-nearest neighbor ($k$NN) algorithm
% \cite{MLkNN_ALazyLearningApproach}. It finds the $k$ nearest neighborhood of an
% input instance using $k$NN, then uses Bayesian inference to determine the label
% set of the instance. We studied this method because it has been reported to
% achieve considerable performance for different multi-label classification tasks
% in previous studies \cite{MLkNN_ALazyLearningApproach,
% mlknn_MultilabelTextClassificationUsingSemanticFeatures}. We used ML-$k$NN with
% the number of nearest neighbors, $K$ = 10 during our experiment as recommended
% by \cite{mlknn_MultilabelTextClassificationUsingSemanticFeatures}.
% 
% \end{inparaenum}

\subsubsection{Studied Features}
We used two types of features: (1) rule-based metrics (described in Section
\ref{subsubsec:rule-based-metrics}) and (2) bag of words (BoW) \cite{bag_of_words_paper_1}. Bag of words (BoW) is a common feature extraction
procedure for text data and has been successfully used for text classification
problems \cite{bag_of_words_for_text_1,bag_of_words_for_text_2}.

%use two types of features: the rule-based metrics, bag-of-words (as a proxy of word embeddings which will be used in BERT/LSTM - you need to ensure that reviewers are convinced that you have looked at each option before claiming BERT is a the best classifier)

%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}


\begin{table*}[t]
\caption{Class-wise performance of shallow machine learning models}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{p{.75cm}|lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Feature}}   & {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
\multirow{5}{=}{\textbf{Rule Based Feats}}  
%&  {\textbf{Baseline}}  
%& {.77} & {.69} & {.86} &{.76} %bloated
%& {.58} & {.69} & {.71} &{.70} %lazy
%& {.75} & {.37} & {.50} &{.42} %excess
%& {.49} & {.41} & {.39} &{.40} %tangled
%& {.65} & {.58} & {.60} &{.59} %fragmented
%\\ %\hline
& {\textbf{OVR-SVM}} 
& {.96} & {.88} & {.89} & \bf{.88} %bloated
& {.94} & {.86} & {.94} &{.90} %lazy
& {.74} & {.45} & {.23} &{.31} %excess
& {.82} & {.67} & {.56} &\bf{.61} %tangled
& {.80} & {.69} & {.25} &{.37} %fragmented
\\ %\hline
& {\textbf{LPS-SVM}} 
& {.94} & {.86} & {.70} &{.77} %bloated
& {.91} & {.77} & {.97} &{.86} %lazy
& {.74} & {.44} & {.21} &{.28} %excess
& {.80} & {.70} & {.40} &{.51} %tangled
& {.81} & {.73} & {.32} &{.45} %fragmented
\\ %\hline
& {\textbf{CC-SVM}}  
& {.96} & {.88} & {.87} &\bf{.88} %bloated
& {.92} & {.79} & {.97} &{.87} %lazy
& {.75} & {.47} & {.24} &{.32} %excess
& {.82} & {.68} & {.54} &{.60} %tangled
& {.80} & {.71} & {.27} &{.39} %fragmented
\\ %\hline
& {\textbf{ML-$k$NN}}  
& {.93} & {.73} & {.89} &{.80} %bloated
& {.91} & {.86} & {.80} &{.83} %lazy
& {.75} & {.49} & {.31} &{.38} %excess
& {.80} & {.63} & {.54} &{.58} %tangled
& {.79} & {.57} & {.50} &{.53} %fragmented
\\ %\hline
\midrule

\multirow{4}{=}{\textbf{BoW Feats}}
& {\textbf{OVR-SVM}}
& {.93} & {.84} & {.66} &{.74} %bloated
& {.95} & {.87} & {.96} &\bf{.91} %lazy
& {.75} & {.49} & {.47} &{.48} %excess
& {.78} & {.57} & {.54} &{.56} %tangled
& {.79} & {.55} & {.54} &{.55} %fragmented
\\%\hline
& {\textbf{LPS-SVM}}
& {.93} & {.89} & {.63} &{.74} %bloated
& {.94} & {.83} & {.97} &{.89} %lazy
& {.75} & {.50} & {.49} &\bf{.50} %excess
& {.79} & {.59} & {.58} &{.58} %tangled
& {.80} & {.59} & {.58} &\bf{.58} %fragmented
\\ %\hline
& {\textbf{CC-SVM}}
& {.93} & {.85} & {.67} &{.75} %bloated
& {.94} & {.85} & {.96} &{.90} %lazy
& {.74} & {.48} & {.47} &{.48} %excess
& {.78} & {.57} & {.54} &{.56} %tangled
& {.78} & {.54} & {.54} &{.54} %fragmented
\\ %\hline
& {\textbf{ML-$k$NN}}
& {.93} & {.86} & {.60} &{.71} %bloated
& {.88} & {.75} & {.83} &{.79} %lazy
& {.73} & {.44} & {.29} &{.35} %excess
& {.79} & {.59} & {.53} &{.56} %tangled
& {.80} & {.63} & {.41} &{.50} %fragmented
\\ %\hline
\bottomrule
%{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
%{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
%\hline
\end{tabular}
%}
\label{table_individual_performance_shallow}
%\end{center}
\end{table*}
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%

Table \ref{table_individual_performance_shallow} presents the performance of the
shallow learning models. The best performer is OVR-SVM, followed closely by CC-SVM. CC-based
models are generally superior to OVR-based models because of the capability of
capturing label correlation \cite{CC_2_ClassifierChainsForMultilabel}. Since the
labels (types) of the presentation smells are not correlated (see 
\sec\ref{sec:benchmark-details}), the CC-based SVM could not
exhibit higher performance than the OVR-based SVM. Using rule-based features, OVR-SVM achieved a
higher F1-score (0.88) than the other models for bloated documentation
detection. Because documentation length (a rule-based) was more effective in
detecting bloated documentation than bag of words. On the other hand, LPS-SVM
achieved a higher F1-score (0.58) for fragmented documentation detection using
bag of words, as bag of words more successfully determined whether the
documentation was referring to other documentation than any rule-based features.
Overall, the shallow
models outperformed the rule-based classifiers for four smell types (except for
lazy documentation smell). Therefore, the documentation
smell detection does not normally depend on a single rule-based metric, rather, it depends
on a combination of different metrics and their thresholds. The shallow learning
models attempted to capture this combination of thresholds, and therefore,
achieved better performances than the baseline models.


\subsubsection{Feature Importance Analysis}
We verified the importance of our rule-based features by applying 
permutation feature importance technique \cite{permutation_feature_importance_paper_1,
permutation_feature_importance_paper_2} in the
best performing shallow model, i.e., OVR-SVM. We first train OVR-SVM with all
the features. While testing, we randomly shuffle the values
of one feature at a time while keeping other feature
values unchanged. A feature is important if shuffling its
values affects the model performance. We calculate the
change in performance in two ways. First, we measure the change in the
average F1-score of the OVR-SVM model for the permutation of a feature. Second,
we report the change of the specific class that the feature
was intended for (i.e., `Documentation  Length' for `Bloated'). We observe that
the permutation of any of our rule-based features degrades the model performance (see Table
\ref{table:permutation_feature_importance}). For example, after permutation of the
values of the `Documentation Length' of test data, the average F1-score
decreases by 0.17 (from 0.62 to 0.45) and the F1-score of the desired class
(i.e., `Bloated') decreases by 0.46 (from 0.88 to 0.42). This analysis
confirms the importance of combining rule-based metrics as features in the models.


% \begin{table}
% \centering
% \caption{OVR-SVM performance decrease in feature permutation}
% \begin{tabular}{lccc}
% \toprule
% \textbf{\begin{tabular}[l]{@{}c@{}}\ \textbf{Permutated} \\   \textbf{Feature}\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}\ \textbf{Intended} \\   \textbf{Class}\end{tabular}} &
% \textbf{\begin{tabular}[c]{@{}c@{}}Decrease in \\ Avg. F1\end{tabular}} &
% \textbf{\begin{tabular}[c]{@{}c@{}}Decrease in \\ F1 of \\ intended \\ class\end{tabular}} \\ \midrule
%  {Doc Length} &  {Bloated}                      & {.17}          & {.46}            \\ %\hline
%  {Readability} & {Tangled}                      & {.06}          & {.11}                   \\ %\hline
%  {\#Acronym\&Jargon} & {Tangled}                & {.05}          & {.07}                   \\ %\hline
%  {\#URLs } & {Fragmented}                       & {.03}          & {.11}                   \\ %\hline
%  {\#Method,Class,Package} & {Excess Struct}     & {.17}          & {.08}                   \\ %\hline
%  {Edit Distance} & {Lazy}                       & {.09}          & {.37}                   \\
% \bottomrule
% \end{tabular}
% %}
% \label{table:permutation_feature_importance}
% %\end{center}
% \end{table}

\begin{table}
\centering
\caption{OVR-SVM performance decrease in feature permutation}
\begin{tabular}{llrr}
\toprule
\bf{Permuted} & \bf{Desired} & \multicolumn{2}{c}{\bf{Decrease in F1}}\\ \cline{3-4}
\bf{Feature} &  \bf{Class C} & \bf{Overall} & \bf{Desired C} \\ 
\midrule 
%\textbf{\begin{tabular}[l]{@{}c@{}}\ \textbf{Permutated} \\   \textbf{Feature}\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}\ \textbf{Intended} \\   \textbf{Class}\end{tabular}} &
%\textbf{\begin{tabular}[c]{@{}c@{}}Decrease in \\ Avg. F1\end{tabular}} &
%\textbf{\begin{tabular}[c]{@{}c@{}}Decrease in \\ F1 of \\ intended \\ class\end{tabular}} \\ \midrule
 Doc Length &  {Bloated}                      & {.17}          & {.46}            \\ %\hline
 Readability & {Tangled}                      & {.06}          & {.11}                   \\ %\hline
 \#Acronym\&Jargon & {Tangled}                & {.05}          & {.07}                   \\ %\hline
 {\#URLs } & {Fragmented}                       & {.03}          & {.11}                   \\ %\hline
 \#Method, Class, Package & {Excess Struct}     & {.17}          & {.08}                   \\ %\hline
 Edit Distance & {Lazy}                       & {.09}          & {.37}                   \\
\bottomrule
\end{tabular}
%}
\label{table:permutation_feature_importance}
\vspace{-.5cm}
%\end{center}
\end{table}
\begin{table*}[t]
\caption{Class-wise performance of deep learning models}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{p{.75cm}|lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}&  \multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Feature}}   & {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\ \textbf{Word} \\   \textbf{Embed}\end{tabular}}
&{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
&{\textbf{BERT}}    & {.93} & {{.93}} & {{.93}} &{\textbf{.93}} & {{.97}} & {{.97}} & {{.97}} &{\textbf{.97}} & {.76} & {{.75}} & {{.76}} &{\textbf{.76}} & {.83} & {{.83}} & {{.83}} &{\textbf{.83}} & {.75} & {.75} & {{.75}} &{\textbf{.75}} \\ 
\bottomrule
\end{tabular}
%}
\label{table_individual_performance_deep}
%\end{center}
\end{table*}

% feature ablation study (rough)
%permutated feature  -    overall f1    -  specific label f1
%  -------------           ---------        -------------
%  	doc_len			-	  0.45 (0.62)  -     0.42  (bloated: 0.88)
%  readability		-	  0.56 (0.62)  -     0.50  (tangled: 0.61)
% acronym+jargon		-	  0.57 (0.62)  -     0.54  (tangled: 0.61)
%      URL           -     0.59 (0.62)  -     0.26  (fragmented: 0.37)
%method,class,package-     0.45 (0.62)  -     0.23  (excess struct: 0.31)
%  edit distance     -     0.53 (0.62)  -     0.53  (lazy: 0.90)




\subsection{Performance of Deep Learning Models (RQ5)}\label{sec:deep-learning}
\subsubsection{Deep Learning Models}
We evaluated two deep learning models, Bidirectional LSTM (Bi-LSTM) and
Bidirectional Encoder Representations from Transformers (BERT).
We picked {Bi-LSTM}, because it is more capable of exploiting contextual information than the
unidirectional LSTM \cite{bilstm_FramewisePhonemeClassificationWithBiLSTM}.
Hence, the Bi-LSTM network can detect the documentation smell by capturing the
information of the API documentations from both directions. BERT is a  pre-trained model which was
designed to learn contextual word representations of unlabeled texts
\cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. We picked BERT, because it is found to significantly outperform 
other models in various natural language processing and text
classification tasks
\cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}.
We constructed a
Bi-LSTM model with 300 hidden states. We used ADAM optimizer
\cite{adam_optimizer} with an initial learning rate of 0.001. We trained the
model with batch size 256 over 10 epochs. 
We used BERT-Base for this study which has 12 layers with 12 attention heads and
110 million parameters. We trained it on benchmark for 10 epochs with
a mini-batch size of 32. We used early-stop to avoid overfitting
\cite{early_stop_bert_1} and considered validation loss as the metric of the
early-stopping \cite{early_stop_bert_2}. The maximum length of the input
sequence was set to 256. We used AdamW optimizer \cite{adam_w} with the learning
rate set to 4e\textsuperscript{-5}, $\beta1$ to 0.9, $\beta2$ to 0.999, and $\epsilon$ to
1e\textsuperscript{-8}
\cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers,
bert_fine_tuning}. We used binary cross-entropy to calculate the loss
\cite{binary_cross_AreLossFunctionSame}.


% \begin{inparaenum}[(a)]
% \item\bf{Bidirectional LSTM (Bi-LSTM)} is more capable of exploiting contextual information than the unidirectional LSTM \cite{bilstm_FramewisePhonemeClassificationWithBiLSTM}. Hence, the Bi-LSTM network can detect the documentation smell by capturing the information of the API documentations from both directions. We constructed a Bi-LSTM model with 300 hidden states. We used ADAM optimizer \cite{adam_optimizer} with an initial learning rate of 0.001. We trained the model with batch size 256 over 10 epochs.
% 
% %\subsubsection{LPS-SVM}
% %\label{subsubsec:lps_svm}
% \item\bf{Bidirectional Encoder Representations from Transformers (BERT)} is a  pre-trained model which was designed to learn contextual word representations of unlabeled texts \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. Considering the great success of BERT in various natural language processing and text classification tasks \cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}, we feel motivated to evaluate its’ performance in documentation smell detection. We used BERT-Base for this study which has 12 layers with 12 attention heads and 110 million parameters. We trained it on our labeled dataset for 10 epochs with a mini-batch size of 32. We used early-stop to avoid overfitting \cite{early_stop_bert_1} and considered validation loss as the metric of the early-stopping \cite{early_stop_bert_2}. The maximum length of the input sequence was set to 256. We used AdamW optimizer \cite{adam_w} with the learning rate set to 4e\textsuperscript{-5}, ß1 to 0.9, ß2 to 0.999, and epsilon to 1e\textsuperscript{-8} \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers, bert_fine_tuning}. We used binary cross-entropy to calculate the loss \cite{binary_cross_AreLossFunctionSame}.
% 
% \end{inparaenum}




 


\subsubsection{Studied Features}
We used word embedding as feature which
is a form of word representation that is capable of capturing the context of a
word in a document by mapping words with similar meaning to a similar
representation. For Bi-LSTM, we used 100-dimensional pre-trained GloVe embedding
which was trained on a dataset of one billion tokens (words) with a vocabulary
of four hundred thousand words \cite{Glove_GlobalVectorsForWordRepresentation}. We used the pre-trained embedding in BERT model \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}.


\subsubsection{Results}


%On the other hand, Bi-LSTM and BERT
%focused on capturing generalized attributes for each smell type and as a result,
%achieved impressive performance in all the performance metrics. Overall, BERT
%showed promising results among all the models in accurately detecting each of
%the individual documentation smells.
%\begin{table}
%\caption{Overall performance of deep learning models}
%\begin{tabular}{c|lcc}
%\toprule
%{\textbf{Feature}} & \textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule
%\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\ \textbf{Word} \\   %\textbf{Embeddings}\end{tabular}}
%&\textbf{Bi-LSTM} & .43                        & .17                   \\ %\hline
%&\textbf{BERT}    & \textbf{.53}               & .14                   \\ %\hline
%\bottomrule
%\end{tabular}
%}
%\label{table_overall_performance_deep}
%\end{center}
%\end{table}

% \begin{table*}[!ht]
% \caption{Performance on different type of documentation smells}
% \begin{center}
% \scalebox{1.0}
% {
% %\renewcommand*{\arraystretch}{3}
% \begin{tabular}{ccccccccccccccccccccc}
%                                        & \multicolumn{20}{c}{}                                         \\ \cline{2-21} 
%{}                  & \multicolumn{4}{c|}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c|}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c|}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c|}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c|}{\textbf{Fragmented}}                                                                  \\ \hline
% {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ \hline
% %{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
% %{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
% %{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
% %{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
% %{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
% {\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
% {\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ \hline
% \end{tabular}
% }
% \label{table_individual_performance}
% \end{center}
% \end{table*}

Table \ref{table_individual_performance_deep} shows the performance of the deep
learning models. BERT outperformed
Bi-LSTM, the shallow, and rule-based classifiers to detect each smell (F1-score). 
{The increase in F1-score in BERT compared to the best performing shallow learning model per smell is as follows: bloated (5.7\% over OVR-SVM Rule), 
lazy (6.6\% over OVR-SVM BoW), Excess Structural Information (52\% over ML-kNN BoW), tangled (36.1\% over OVR-SVM Rule), and 
fragmented (36.4\% over OVR-SVM BoW).} SVM and kNN-based models produced
more false-negative results because the number of positive instances for an
individual smell type is lower than the number of negative
instances for that type. As a result, SVM and kNN-based models showed low
recalls for some types (Excess structural information, Tangled, and Fragmented) and
consequently resulted in low F1-scores. On the other hand, Bi-LSTM and BERT achieved better performance because they
focused on capturing generalized attributes for each smell type. We manually analyzed the misclassified examples of Excess Structural Information and
fragmented documentation where BERT achieved below 0.8 accuracy. For the
Excess Structural Information smell detection, BERT falsely considered some java objects and
methods as structural information; therefore, the model produced some false
positive cases. In some examples, BERT could not identify whether the
information of documentation was referring to other documentation. As a result,
the model misclassified the fragmented documentation.



==> DocBotSANER2021 (Camera Ready)/study-setup.tex <==
\section{Benchmark Study of the Five API Documentation Smells}
% \begin{figure*}[t]%[!htb]
%   \centering
%   %\vspace{-6mm}
%    \hspace*{-.7cm}%
%   \includegraphics[scale=.6]{new_images/FlowChartDocSmell.png}
%  % \vspace{-4mm}
%   \caption{Workflow of our study.}
% 
%   \label{fig:workflow_of_study}
% %\vspace{-4mm}
% \end{figure*}
We answer the following three research questions:

\begin{enumerate}[label=RQ\arabic{*}, leftmargin=25pt]
  \item How accurate are shallow machine learning models to automatically detect the documentation smells?
  \item Can the deep machine learning models outperform the shallow learning models to detect the documentation smells?
  \item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}


%\subsection{Performance Metrics}
We analyze and report the performance of each of the techniques developed and experimented as part of the algorithms development steps. We used 5-fold iterative stratified cross-validation for reporting performances that has been recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}. We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

\nd\bf{Iterative Stratified Cross-Validation}
Traditional $k$-fold cross-validation is a statistical method of evaluating machine learning algorithms which divides data into $k$ equally sized folds and runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each iteration, each of the $k$ folds is used as the held-out set for validation while the remaining $k-1$ folds are used as training sets. Stratified cross-validation is used to make sure that each fold is an appropriate representative of the original data by producing folds where the proportion of different classes is maintained \cite{stratified_cross_validation_paper}. However, stratification is not sufficient for multi-label classification problems as the number of distinct labelsets (i.e., different combinations of labels) is often quite large. For example, there can be 32 combinations of labels in our study as there are 5 types of documentation smells. In such cases, original stratified $k$-fold cross-validation is impractical since most groups might consist of just a single example. Iterative stratification, proposed by \cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy approach of selecting the rarest groups first and adding them to the smallest folds while splitting. Hence, we used this iterative stratified cross-validation in our experiment. 

\nd\bf{Exact Match Ratio}
In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

\begin{equation}
EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
\label{eq:EMR}
\end{equation} %&

{$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
}


\nd\bf{Hamming Loss}
Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
\begin{equation}
HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
\end{equation}

{$N$ is the total number of data, $L$ is the total number of labels.}

\nd\bf{Accuracy}
Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
\begin{equation}
A = \frac{TP+TN}{TP+FN+TN+FP}
\label{eq:acc}
\end{equation}

{$TP$ is the number of true positives, $FN$ is the number of false
negatives, $FP$ is the number of false positives, $TN$ is the number of true
negatives.}


\nd\bf{Precision}
Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
\begin{equation}
P  = \frac{TP}{TP+FP} 
\label{eq:precision}
\end{equation} %&


\nd\bf{Recall}
Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

\begin{equation}
 R = \frac{TP}{TP+FN}
 \label{eq:recall}
 \end{equation} 
 

\nd\bf{F1-score}
F1-score is the harmonic mean of precision and recall.
\begin{equation}
F1 = \frac{2\cdot P\cdot R}{P+R}
\label{eq:f-score}    
\end{equation}






==> DocBotSANER2021 (Camera Ready)/survey.tex <==
\section{Developers' Survey of Documentation Smells}\label{sec:survey}
Four out of the five API documentation smells in our study were previously reported as commonly observed by 
IBM developers~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 
The other smell (lazy documentation) is reported as a problem in API documentation in multiple studies~\cite{Aghajani-SoftwareDocPractitioner-ICSE2020,Robillard-APIsHardtoLearn-IEEESoftware2009a}. 
Given that we extended previous studies by creating a benchmark of the smells with real-world examples, we needed to further 
ensure that our collected examples of smelly documentation units do resonate with 
software developers. We, therefore, conducted a survey of professional software developers (1) to validate our catalog of the five API documentation smells and (2) to 
understand whether, similar to previous research, developers agree with the negative impact of the documentation smells. In particular, 
we explore the following two research questions:
\begin{enumerate}[label=RQ\arabic{*}., leftmargin=25pt]
  \item How do software developers agree with our catalog and examples of the five API documentation smells?
  \item How do software developers perceive the impact of the detected documentation smells?
\end{enumerate}\subsection{Survey Setup}
We recruited 21 professional software developers who are working in the software industry. 
We ensured that each developer is actively involved in daily software development activities like API reuse and documentation 
consultation. The participants were collected through personal contacts. First, each participant had to answer two demographic questions: current profession and years of experience in software development. 
We then presented each participant two Javadoc examples
of each smell and asked him/her whether they agreed that this documentation example
belonged to that particular smell. Then, we asked them about how frequently they
faced these documentation smells. Finally, we inquired them of the negative impact of the documentation smells on their overall productivity during software development. 
Out of the 21 participants, 14 participants had
experience less than 5 years and the rest had more than 5 years. Majority of the
participants had experience less than 5 years because they are likely to be more engaged in studying API documentation as part of their software programming 
responsibility. Developers with experience more than five years are more engaged in design of the software and its architecture.


\begin{figure}[t]%[!htb]
  \centering
  
  \includegraphics[scale=.4]{new_images/survey_examples.png}

  \caption{Survey response on whether the software developers agreed with our labeled documentation smell examples.}

  \label{fig:survey_examples}

\end{figure}
\begin{figure}[t]
  \centering
  
  \includegraphics[scale=.4]{new_images/survey_frequency.png}

  \caption{Survey response on how frequently the participants faced the documentation smells in the last three months.}

  \label{fig:survey_frequency}

\end{figure}

\subsection{How do software developers agree with our catalog and examples of the five API documentation smells? (RQ1)}
We showed each participant two examples of each smell, i.e., 10 examples in total. For each example, we asked 
two questions: (1) Do you think the documentation mentioned above is [smell, e.g., lazy]? The options are in Likert scale, i.e., strongly agree, agree, neutral, disagree, and strongly disagree. 
and (2) Based on your experience 
of the last three months, how frequently did you observe this [smell, e.g., lazy] in documentation? 
The options are: never, once or twice, occasionally, frequently, and no opinion. The options are picked from literature \cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 
Two examples per smell ensure increased 
confidence on the feedback we get from each participant.

\fig\ref{fig:survey_examples}
shows the responses of the participants to the first question. More than 75\% participants agreed to the examples of three smells: bloated, tangled, and 
excess structural info. At least 50\% of the participants agreed to the examples of the other two smells. Only 5-25\% of the participants 
disagreed to the examples. Overall, each example of the API documentation smell was agreed by at least 50\% of the participants. This validates 
out catalog of API documentation smells based on feedback from the professional developers. 
%that the examples and documentation smells resonated with the participants.\anindya{The last line does not carry clear meaning.}

\fig\ref{fig:survey_frequency} shows the frequency of the documentation
smells the developers observed in the last three months (second question). We found that 50\% of
the participants had faced all the smells and lazy smell was the most
frequently encountered. On the other hand, half
of the participants did not face bloated documentation smells in the last three
months, while 60\%-65\% of the participants faced tangled, excess structural info,
and fragmented API documentation. This study reveals that API documentation is
becoming less explicable, more complex, and unnecessarily structured to keep the
documentation short. To solve this problem, API documentation
needs to be more understandable and elaborated to explain the API functionality.

\subsection{How do software developers perceive the impact of the detected documentation smells? (RQ2)}
We asked the participants how severely the documentation smells impact their
development tasks. The responses were taken on a scale of five degrees:
"Blocker", "Severe", "Moderate", "Not a Problem", and "No opinion". The options were picked from similar questions 
on API documentation presentation problems from literature~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}.
\begin{figure}[!htb]
  \centering
  
  \includegraphics[scale=.5]{new_images/survey_severity_2.png}

  \caption{The perceived impact of the five documentation smells by severity and frequency. Circle size indicates the 
  percentage of participants who strongly agreed or agreed to the smells.}

  \label{fig:survey_severity}

\end{figure}

We analyzed the impact of the documentation smells with respect to the
frequency of the smells the participants had observed over the past three months (see \fig\ref{fig:survey_severity}). 
For each smell, we compute the frequency scale (x-axis) as the percentage of
response "Frequently", "Occasionally", and "Once or twice". For example, regarding whether the participants had
observed lazy documentation in the past three months, 25\% answered
"Frequently", 35\% answered "Occasionally", and 30\% answered "Once or twice",
leading to a total  90\% in the frequency scale. We constructed the severity
scale (y-axis) by combining the percentage of the participants responded with "Blocker",
"Severe", and "Moderate". For
example, due to fragmented documentation smells, 5\% of the participants could
not use that particular API and picked another API ("Blocker"), 20\% of the
participants believed that they wasted a lot of time figuring out the API
functionality ("Severe"), and 25\% of the participants felt irritated
("Moderate") with the fragmented documentation. The circle size indicates the
percentage of the participants "Strongly Agree" or "Agree" with the examples
containing documentation smells.

From \fig\ref{fig:survey_severity}, we observed that lazy documentation had
the most frequent and the most negative impact (90\%). Tangled documentation was
identified as the second most severe smell (85\%). Although bloated
documentation was considered more severe (65\%) than excess structural info (55\%
severity) and fragmented (50\% severity) documentation, bloated occurred less
frequently than the later two. The most important finding of this survey is that
the coordinates of all the circles (referring to documentation smells) in \fig\ref{fig:survey_severity} were above or equal to 50. This indicates that
according to the majority of the participants, these documentations smells are
occurring frequently and hindering the productivity of the development tasks.



==> DocBotSANER2021 (Camera Ready)/threats.tex <==
\section{Threats to Validity}
%threats to validity
In this work, we conducted our experiments on a relatively small dataset. Since, to the best of our knowledge, detecting the documentation smells is the first of its kind, we manually labeled a small portion of the Java API documentation due to the time constraint. However, we randomly sampled the documentations for manual labeling, therefore, we expect that the actual distributions of the documentation smells will remain identical in case of adding more documentation examples. Furthermore, we performed cross-validation on our dataset to reduce the effect of any non-representative subset. The number of participants in our survey is too low to get a clear picture of how the documentation smells affect productivity on the large scale. We conducted the survey with an aim to validate the catalog we developed by the software developers. As the developers agreed with the catalog and its negative impact on the productivity, in the future extension of this study, we can include more participants to categorize the documentations into different documentation smells based on this catalog.


==> backup/study_result_backup.tex <==
\section{Automatic Detection of The Smells}
We answer the following four research questions:

\begin{enumerate}[label=RQ\arabic{*}., leftmargin=25pt]
  \item How accurate are rule-based classifiers to automatically detect the documentation smells?
  \item Can the shallow machine learning models outperform the rule-based classifiers?
  \item Can the deep machine learning models outperform the shallow learning models?
  \item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}
\subsection{Performance Metrics}
We analyze and report the performance of each of the techniques developed and experimented as part of the algorithms development steps. We used 5-fold iterative stratified cross-validation for reporting performances that has been recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}. We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

\begin{inparaenum}[(a)]
\item\bf{Iterative Stratified Cross-Validation}
Traditional $k$-fold cross-validation is a statistical method of evaluating machine learning algorithms which divides data into $k$ equally sized folds and runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each iteration, each of the $k$ folds is used as the held-out set for validation while the remaining $k-1$ folds are used as training sets. Stratified cross-validation is used to make sure that each fold is an appropriate representative of the original data by producing folds where the proportion of different classes is maintained \cite{stratified_cross_validation_paper}. However, stratification is not sufficient for multi-label classification problems as the number of distinct labelsets (i.e., different combinations of labels) is often quite large. For example, there can be 32 combinations of labels in our study as there are 5 types of documentation smells. In such cases, original stratified $k$-fold cross-validation is impractical since most groups might consist of just a single example. Iterative stratification, proposed by \cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy approach of selecting the rarest groups first and adding them to the smallest folds while splitting. Hence, we used this iterative stratified cross-validation in our experiment. 

\item\bf{Exact Match Ratio}
In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

\begin{equation}
EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
\label{eq:EMR}
\end{equation} %&

{$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
}


\item\bf{Hamming Loss}
Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
\begin{equation}
HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
\end{equation}

{$N$ is the total number of data, $L$ is the total number of labels.}

\item\bf{Accuracy}
Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
\begin{equation}
A = \frac{TP+TN}{TP+FN+TN+FP}
\label{eq:acc}
\end{equation}

{$TP$ is the number of true positives, $FN$ is the number of false
negatives, $FP$ is the number of false positives, $TN$ is the number of true
negatives.}


\item\bf{Precision}
Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
\begin{equation}
P  = \frac{TP}{TP+FP} 
\label{eq:precision}
\end{equation} %&


\item\bf{Recall}
Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

\begin{equation}
 R = \frac{TP}{TP+FN}
 \label{eq:recall}
 \end{equation} 
 

\item\bf{F1-score}
F1-score is the harmonic mean of precision and recall.
\begin{equation}
F1 = \frac{2\cdot P\cdot R}{P+R}
\label{eq:f-score}    
\end{equation}

\end{inparaenum}

\subsection{ How accurate are rule-based classifiers to automatically detect the documentation smells? (RQ1)}
\subsubsection{Rule-based Metrics}
%\subsubsection{Approach}
%\gias{discuss the studied features, put the feature summaries in a table}
%discuss the features, group the features into a set of feature dimensions.


\begin{inparaenum}[(a)]
\item\bf{Documentation Length.} We use the length of every documentation in order to capture the extensiveness of the bloated documentations.

\item\bf{Readability Metrics.} We measure Flesch readability metrics for the documentations and use them as a feature to analyze the understandability of documentation. This feature might be useful to detect tangled documentations.

\item\bf{Number of Acronyms and Jargons.} Since acronyms and jargons increase the complexity of a reading passage, we use the number of acronyms and jargon in every documentation to detect the tangled documentation by estimating the understandability.

\item\bf{Number of URLs.} As URLs are hints of possible fragmentations in the documentation, we use the number of URLs to capture these smells.

\item\bf{Number of function, class and package name mentioned.} We use the number of functions, classes, packages mentioned in documentation to capture excess structural information and fragmentation.

\item\bf{Edit Distance.} From the definition of lazy documentation, it can be said that the edit distance of a lazy documentation and its’ unit definition (method prototype) will be comparatively small. So we calculate the edit distance between the documentation description and method prototype and use it as a feature for our machine learning models.

\item\bf{Average Cosine Similarity.} We calculate the avg. cosine similarity of the documentations’ description. For this, we calculate the cosine similarities between each possible pair of that documentation and take their avg value for normalization. This feature will help to detect redundancy in the documentations.
\end{inparaenum}

\subsubsection{Results}
discuss the results by varying the metric thresholds

\subsection{How accurate are shallow machine learning models to automatically detect the documentation smells? (RQ2)}
\subsubsection{Shallow Learning Models}
We applied both traditional and deep learning algorithms to detect documentation smells. We employed different decomposition approaches (i.e., One-Vs-Rest, Label Powerset, Classifier Chains)~\cite{multilabel_decomp_1_MultilabelClassificationAnOverview,multilabel_decomp_2_AReviewOnMultilabelLearning,multilabel_decomp_3_ATutorialOnMultilabelClassification,multilabel_decomp_4_LearningFromMultilabelData} with Support Vector Machine (SVM) \cite{SVM_SupportVectorNetworks} as the base estimator for multi-label classification of documentation smells. We chose SVM since it has been successfully used with these decomposition approaches for multi-label classification in previous studies \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}. SVM has also shown great performance in text classification tasks \cite{svm_text_classification_1, svm_text_classification_2}. We also evaluated adapted approaches like ML-$k$NN \cite{MLkNN_ALazyLearningApproach}, and deep learning models like Bi-LSTM \cite{bi_lstm_BidirectionalRecurrentNeuralNetworks}, and BERT \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. 

%\subsubsection{OVR-SVM}
%\label{subsubsec:ovr_svm}
\begin{inparaenum}[(a)]
\item\bf{One-Vs-Rest} is a heuristic method that works by decomposing the multi-label classification problem into multiple independent binary classification problems (one per class) \cite{multilabel_decomp_1_MultilabelClassificationAnOverview, multilabel_decomp_3_ATutorialOnMultilabelClassification}. It trains a single classifier per class, with the samples of that class as positive samples and all other samples as negatives. All the independent classifiers then separately give individual class predictions for unseen data. We evaluated One-Vs-Rest (OVR) approach with SVM (as the base estimator) for detecting documentation smells. One-Vs-Rest support vector machine (OVR-SVM) has been successfully applied in several problems \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM, multilabel_decomp_1_MultilabelClassificationAnOverview}. We used RBF kernel for the SVM classifiers as recommended by earlier works \cite{svm_rbf_1_AComparisonStudyOfDifferentKernelFunctions, svm_rbf_2_APracticalGuideToSVM}.

%\subsubsection{LPS-SVM}
%\label{subsubsec:lps_svm}
\item\bf{Label Power Set (LPS)} treats every combination of labels as a new class and approaches in a multiclass classification manner \cite{LearningMultiLabelSceneClassification}. As a result, this method has high computational complexity. However, it is capable of taking label correlation into account. We used SVM (with RBF kernel) as the base estimator of the Label Power Set method \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}.


%\subsubsection{CC-SVM}
%\label{subsubsec:cc_svm}
\item\bf{Classifier Chains (CC)} constructs a chain of binary classifiers, where every classifier uses the predictions of all the previous classifiers of the chain \cite{CC_1_ClassifierChainsForMultilabel, CC_2_ClassifierChainsForMultilabel}. This way the method can take label correlations into account. We constructed a Classifier Chain (CC) of SVMs and evaluated its’ performance for documentation smell detection.



%\subsubsection{ML-$k$NN}
%\label{subsubsec:ml_knn}
\item\bf{Multi-label $k$ Nearest Neighbors (ML-$k$NN)} is derived from the traditional $k$-nearest neighbor ($k$NN) algorithm \cite{MLkNN_ALazyLearningApproach}. It finds the $k$ nearest neighborhood of an input instance using $k$NN, then uses Bayesian inference to determine the label set of the instance. We studied this method because it has been reported to achieve considerable performance for different multi-label classification tasks in previous studies \cite{MLkNN_ALazyLearningApproach, mlknn_MultilabelTextClassificationUsingSemanticFeatures}. We used ML-$k$NN with the number of nearest neighbors, $K$ = 10 during our experiment as recommended by \cite{mlknn_MultilabelTextClassificationUsingSemanticFeatures}.

\end{inparaenum}

\subsubsection{Studied Features} In this subsection, we describe the features that we used to train our SVM and \it{k}NN-based models (see section \ref{subsubsec:ovr_svm} to \ref{subsubsec:ml_knn}) for documentation smell detection.

use two types of features: the rule-based metrics, bag-of-words (as a proxy of word embeddings which will be used in BERT/LSTM - you need to 
ensure that reviewers are convinced that you have looked at each option before claiming BERT is a the best classifier)

%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}

Table \ref{table_overall_performance} represents the performance of the ML models for detecting documentation smell as a multi-label classification problem. We observe that OneVsRest (OVR) and Classifier Chain (CC) achieved equal results. CC-based models are generally superior to OVR-based models because of the capability of capturing label correlation. Since the labels (types) of the documentation smells are not correlated, the CC-based SVM could not exhibit higher performance than the OVR-based SVM. However, Label Powerset (LPS) achieved lower performance than the OVR and CC-based models. To show better results, LPS-based SVM would require sufficient instances for all 32 classes of 5 smell types. Deep learning-based models like Bi-LSTM and BERT, on the other hand, outperformed the SVM and $k$NN-based models by achieving higher exact match ratios. Although Bi-LSTM showed higher Hamming loss, BERT achieved similar to the SVM and $k$NN-based models. Therefore, in terms of Hamming loss, deep learning-based models did not show any improvement. However, considering both exact match ratio and Hamming loss as the performance metrics, we can deduce that BERT is the most suitable of all the models experimented in detecting the documentation documentation smell.
\begin{table}[t]
\caption{Shallow models on the overall smell types detection}
\centering
%\begin{center}
%\scalebox{1.0}
%\resizebox{\columnwidth}{!} %new add
%{
%\renewcommand*{\arraystretch}{2}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule
\textbf{Rule-based} & .17                        & .35       \\ %\hline
\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
%\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
%\textbf{BERT}    & \textbf{.84}               & .15                   \\ 
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
\bottomrule
%{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
%{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
%\hline
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}
Table \ref{table_individual_performance} shows the performance of the ML models
on each type of documentation smells. Although SVM and $k$NN-based models
achieved slightly better accuracy than Bi-LSTM and BERT, the later models
outperformed SVM and $k$NN-based models in F1-score. This behavior is due to the
unequal distribution of the smell types over the dataset. SVM and $k$NN-based
models produced more false-negative results because the number of positive
instances for an individual smell type is significantly lower than the number of
negative instances for that type. As a result, SVM and $k$NN-based models showed
quite low recalls for some types (Excess Struct, Tangled, and Fragmented) and
consequently resulted in low F1-scores. 
%\subsubsection{Feautre Importance Analysis}
\gias{TODO: do the feature-based analysis here, i.e., ablation study on the shallow learning models as discussed}

\subsection{Can the deep machine learning models outperform the shallow learning models? (RQ3)}
\subsubsection{Deep Learning Models}
%\subsubsection{Bi-LSTM}
Bidirectional LSTM is more capable of exploiting contextual information than the unidirectional LSTM \cite{bilstm_FramewisePhonemeClassificationWithBiLSTM}. Hence, the Bi-LSTM network can detect the documentation smell by capturing the information of the API documentations from both directions. We constructed a Bi-LSTM model with 300 hidden states and initialized it using the pre-trained GloVe embedding \cite{Glove_GlobalVectorsForWordRepresentation} of 100 dimensions. We used ADAM optimizer \cite{adam_optimizer} with an initial learning rate of 0.001. We trained the model with batch size 256 over 10 epochs.


%\subsubsection{BERT}
Considering the great success of BERT (Bidirectional Encoder Representations from Transformers) in various natural language processing and text classification tasks \cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}, we feel motivated to evaluate its’ performance in documentation smell detection. BERT is a  pre-trained model which was designed to learn contextual word representations of unlabeled texts \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. We used BERT-Base for this study which has 12 layers with 12 attention heads and 110 million parameters. We trained it on our labeled dataset for 10 epochs with a mini-batch size of 32. We used early-stop to avoid overfitting \cite{early_stop_bert_1} and considered validation loss as the metric of the early-stopping \cite{early_stop_bert_2}. The maximum length of the input sequence was set to 256. We used AdamW optimizer \cite{adam_w} with the learning rate set to 4e\textsuperscript{-5}, ß1 to 0.9, ß2 to 0.999, and epsilon to 1e\textsuperscript{-8} \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers, bert_fine_tuning}. We used binary cross-entropy to calculate the loss \cite{binary_cross_AreLossFunctionSame}. 


\subsubsection{Studied Features} talk about word-embeddings

\subsubsection{Results}
On the other hand, Bi-LSTM and BERT
focused on capturing generalized attributes for each smell type and as a result,
achieved impressive performance in all the performance metrics. Overall, BERT
showed promising results among all the models in accurately detecting each of
the individual documentation smells.
\begin{table}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule

%\textbf{Rule-based} & .17                        & .35       \\ %\hline
%\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
%\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
%\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
%\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
\textbf{BERT}    & \textbf{.84}               & .15                   \\ %\hline
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}

% \begin{table*}[!ht]
% \caption{Performance on different type of documentation smells}
% \begin{center}
% \scalebox{1.0}
% {
% %\renewcommand*{\arraystretch}{3}
% \begin{tabular}{ccccccccccccccccccccc}
%                                        & \multicolumn{20}{c}{}                                         \\ \cline{2-21} 
%{}                  & \multicolumn{4}{c|}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c|}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c|}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c|}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c|}{\textbf{Fragmented}}                                                                  \\ \hline
% {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ \hline
% %{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
% %{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
% %{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
% %{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
% %{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
% {\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
% {\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ \hline
% \end{tabular}
% }
% \label{table_individual_performance}
% \end{center}
% \end{table*}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
\bottomrule
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
\gias{TODO. Now report some misclassified cases of BERT per documentation smell and explain why the misclassification occurred.}

\subsection{Can the detection of one documentation smell support the detection another smell? (RQ4)}
In multi-label learning, the labels might be interdependent and correlated \cite{label_correlation_paper_1}. We used Phi Coefficients to determine such interdependencies and correlations between different documentation smells. The Phi Coefficient is a measure of association between two binary variables \cite{phi_coefficient_paper}. It ranges from -1 to +1, where ±1 indicates a perfect positive or negative correlation, and 0 indicates no relationship. We report the Phi Coefficients between each pair of labels in Figure \ref{fig:label_correlation}. We find that there is almost no correlation between `Fragmented’ and any other smell (except `Lazy’). By definition, the information of fragmented documentation is scattered in many sections or pages. Hence, it has little to do with smells like `Bloated’, `Excess Structural Information’, `Tangled’. We also observe that there is a weak positive correlation (+0.2 to +0.4) among the `Bloated’, `Excess Structural Information’, and `Tangled’ smells. One possible reason might be that if a documentation is filled with complex and unorganized information (Tangled), and unnecessary structural information (Excess Structural Information), it might be prone to become bloated as well. On the other hand, `Lazy’ smell has a weak negative correlation (-0.2 to -0.3) with all other groups since these kinds of documentation are often too small to contain other smells. However, none of these coefficients is high enough to imply a strong or moderate correlation between any pair of labels. Hence, it justifies our catalog by indicating that all the smells that we proposed are sufficiently unique in nature.

\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
   \hspace*{-.7cm}%
  \includegraphics[scale=.5]{new_images/label_correlation.png}
 % \vspace{-4mm}
  \caption{Correlation of different documentation smells. Red, Blue, and Gray mean positive, negative, and no correlation respectively. Intensity of color indicates the level of correlation.}

  \label{fig:label_correlation}
%\vspace{-4mm}
\end{figure}


% 
% \subsection{Ablation Study (RQ4)}
% BERT - epoch change
% SVM - feature change.



%\subsection{How accurate is each feature dimension?}
%answer RQ

%\subsection{How well does hypertuning work in the ML models?}
%answer RQ.


==> method.tex <==
\section{Methodology}
\begin{figure*}[t]
\centering
	\centering
   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
   	\includegraphics[scale=.85]{images/workflow_mod3}
   	\caption{The five major steps used in this study}
   	 \label{fig:MethodologyOverall}
\vspace{-5mm}
\end{figure*}
While research is devoted to understand code and design smells, we are aware of no previous research on API documentation smells.
Similar to code and design smells that do not directly introduce a defect or a bug into a software system, documentation smells refer to
presentation issues that do not make a documentation incorrect, rather they hinder its proper usage due to the lack of quality in the design 
and presentation of the documented contents. As such, we studied extensively the API documentation literature that reported issues related to 
API documentation presentation and usability~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocIssueUnveiled-ICSE2019}.  
For example, the most recent paper on this topic was by Aghajani et al.~\cite{Aghajani-SoftwareDocIssueUnveiled-ICSE2019,Aghajani-SoftwareDocPractitioner-ICSE2020}, who 
divided the `how' problems in API documentation into four categories: maintainability (e.g., lenghty files), readability (e.g., clarity), 
usability (e.g., information organization), and usefulness (e.g., content not useful in practice). Previously, Uddin and Robillard~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015} 
studied 10 common problems in API documentation by surveying 323 IBM developers. They observed four common presentation problems: bloated (i.e., too long description), 
tangled (complicated documentation), fragmented (i.e., scattered description), and excess structural info (i.e., content not useful in practice). 
Given that the four problems appeared in both studies, we included each as a documentation smell in our study. In addition, we added lack of 
proper description of an API method as a type of `lazy' smell in the documentation, because incomplete documentation problems are 
discussed in both papers~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Aghajani-SoftwareDocPractitioner-ICSE2020} as well as in online developer discussions. 

Once we decided on the five smells, in the 

That this catalog of five smells provides a good starting point to investigate the focus of this paper, i.e., determining the feasbility of automatically detecting 
the smells using automated techniques. To investigate the techniques, we created our benchmark as follows. 


==> study-setup.tex <==
\section{Benchmark Study of the Five API Documentation Smells}
% \begin{figure*}[t]%[!htb]
%   \centering
%   %\vspace{-6mm}
%    \hspace*{-.7cm}%
%   \includegraphics[scale=.6]{new_images/FlowChartDocSmell.png}
%  % \vspace{-4mm}
%   \caption{Workflow of our study.}
% 
%   \label{fig:workflow_of_study}
% %\vspace{-4mm}
% \end{figure*}
We answer the following three research questions:

\begin{enumerate}[label=RQ\arabic{*}, leftmargin=25pt]
  \item How accurate are shallow machine learning models to automatically detect the documentation smells?
  \item Can the deep machine learning models outperform the shallow learning models to detect the documentation smells?
  \item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}


%\subsection{Performance Metrics}
We analyze and report the performance of each of the techniques developed and experimented as part of the algorithms development steps. We used 5-fold iterative stratified cross-validation for reporting performances that has been recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}. We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

\nd\bf{Iterative Stratified Cross-Validation}
Traditional $k$-fold cross-validation is a statistical method of evaluating machine learning algorithms which divides data into $k$ equally sized folds and runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each iteration, each of the $k$ folds is used as the held-out set for validation while the remaining $k-1$ folds are used as training sets. Stratified cross-validation is used to make sure that each fold is an appropriate representative of the original data by producing folds where the proportion of different classes is maintained \cite{stratified_cross_validation_paper}. However, stratification is not sufficient for multi-label classification problems as the number of distinct labelsets (i.e., different combinations of labels) is often quite large. For example, there can be 32 combinations of labels in our study as there are 5 types of documentation smells. In such cases, original stratified $k$-fold cross-validation is impractical since most groups might consist of just a single example. Iterative stratification, proposed by \cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy approach of selecting the rarest groups first and adding them to the smallest folds while splitting. Hence, we used this iterative stratified cross-validation in our experiment. 

\nd\bf{Exact Match Ratio}
In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

\begin{equation}
EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
\label{eq:EMR}
\end{equation} %&

{$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
}


\nd\bf{Hamming Loss}
Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
\begin{equation}
HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
\end{equation}

{$N$ is the total number of data, $L$ is the total number of labels.}

\nd\bf{Accuracy}
Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
\begin{equation}
A = \frac{TP+TN}{TP+FN+TN+FP}
\label{eq:acc}
\end{equation}

{$TP$ is the number of true positives, $FN$ is the number of false
negatives, $FP$ is the number of false positives, $TN$ is the number of true
negatives.}


\nd\bf{Precision}
Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
\begin{equation}
P  = \frac{TP}{TP+FP} 
\label{eq:precision}
\end{equation} %&


\nd\bf{Recall}
Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

\begin{equation}
 R = \frac{TP}{TP+FN}
 \label{eq:recall}
 \end{equation} 
 

\nd\bf{F1-score}
F1-score is the harmonic mean of precision and recall.
\begin{equation}
F1 = \frac{2\cdot P\cdot R}{P+R}
\label{eq:f-score}    
\end{equation}






==> threats.tex <==
\section{Threats to Validity}
%threats to validity
In this work, we conducted our experiments on a relatively small dataset. Since, to the best of our knowledge, detecting the documentation smells is the first of its kind, we manually labeled a small portion of the Java API documentation due to the time constraint. However, we randomly sampled the documentations for manual labeling, therefore, we expect that the actual distributions of the documentation smells will remain identical in case of adding more documentation examples. Furthermore, we performed cross-validation on our dataset to reduce the effect of any non-representative subset. The number of participants in our survey is too low to get a clear picture of how the documentation smells affect productivity on the large scale. We conducted the survey with an aim to validate the catalog we developed by the software developers. As the developers agreed with the catalog and its negative impact on the productivity, in the future extension of this study, we can include more participants to categorize the documentations into different documentation smells based on this catalog.

